Task-space Synergies for Reaching using Upper-limb Prostheses

Synergistic prostheses enable the coordinated movement of the human-prosthetic arm, as required by activities of daily living. This is achieved by coupling the motion of the prosthesis to the human command, such as the residual limb movement in motion-based interfaces. Previous studies demonstrated that developing human-prosthetic synergies in joint-space must consider individual motor behaviour and the intended task to be performed, requiring personalisation and task calibration. In this work, an alternative synergy-based strategy, utilising a synergistic relationship expressed in task-space, is proposed. This task-space synergy has the potential to replace the need for personalisation and task calibration with a model-based approach requiring knowledge of the individual user's arm kinematics, the anticipated hand motion during the task and voluntary information from the prosthetic user. The proposed method is compared with surface electromyography-based and joint-space synergy-based prosthetic interfaces in a study of motor behaviour and task performance on able-bodied subjects using a VR-based transhumeral prosthesis. Experimental results showed that for a set of forward reaching tasks the proposed task-space synergy achieves comparable performance to joint-space synergies without the need to rely on time-consuming calibration processes or human motor learning. Case study results with an amputee subject motivate the further development of the proposed task-space synergy method.

==> DotPointed/discussionDP.tex <==
%
% Discussion
%
\section{Discussion}
\begin{itemize}
    \item Synergistic interfaces allow the coordinated motion required for natural reaching motor behaviour. Subjects that became proficient with these interface within the time allowed for the experiment were able to achieve near-able-bodied movement patterns, showing the capabilities of synergistic interfaces. 
    \item These results suggest that as subjects learned to use the device, they found that the most intuitive, or natural, way of using the prosthetic device was in a similar fashion to able-bodied movements. Whether this was done consciously or subconsciously cannot be determined by the study herein; however, it is an interesting question that remains open for investigation. 
    \item The subjects in the study were all able-bodied, so they were not affected by the changes in motor behaviour experienced by amputees. An important aspect to study is whether the same results are obtained with subjects who have used a prosthetic device for a long time, as their motor behaviour would have significantly changed.
    
    \item The results suggest that the synergy formulation does not significantly impact the outcome of the task or motor behaviour. While JS showed some advantages over TS, the difference was not significant. It appears that subjects were able to internally compensate for the two different mappings (joint-to-joint and joint-to-task), and so were able to use either synergistic interface effectively. TS, however, introduced an additional movement due to the lack of information (object location) required to generate the desired hand path, as such hampering its effectiveness.
    \item These interfaces appear to differ in their learning curve. JS was observed to be easier to use (joint-space to joint-space mapping) while TS was more difficult to use (joint-space to task-space mapping) as seen by the number of subjects that were able to achieve proficiency with the interface, as measured by the motor behaviour metrics. This suggests that the joint-to-task mapping may affect the complexity and intuitiveness of the interface. This could be mitigated by changing how the TS training is provided to subject.
    \item The study only considered short term motor adaptation, and changes in motor behaviour could appear over extended periods of use. Such longitudinal studies will be considered in the later stages of this research.
    
    \item \textbf{Say something about JS not being personalised and future work could look into this?}
    
    \item The simple prosthesis considered in the study may not highlight the advantages of a task-space synergy, as this type of synergy can provide simultaneous control of hand orientation as well which is needed for richer tasks such as drinking. The additional degrees of freedom in the wrist add significant complexity to sEMG interfaces making them even more difficult to use, further motivating the use of synergy. This added complexity will be studied in future work.
\end{itemize}

==> DotPointed/introDP.tex <==
%
% Introduction
%
\section{Introduction}
%
%

%
% Introduce synergies in prosthetics and their advantages.
%
\textbf{Introduce synergies in prosthetics and their advantages.}
\begin{itemize}
    \item Synergistic prosthetic interfaces in upper-limb prostheses enable the coordinated human-prosthetic arm motion required by many activities of daily living.
\end{itemize}

%
% Describe the current method used to realise synergies in transhumeral prosthetics: joint-space synergies
%
\textbf{Describe the current method used to realise synergies in transhumeral prosthetics: joint-space synergies}
\begin{itemize}
    \item The typical realisation of synergies in prosthetic interfaces are joint-space synergies \cite{Kaliki2013, Blana2016, Akhtar2017, Legrand2018, Alshammary2018}. These relate the motion of the joints in the residual limb to a movement of the joints in the prosthetic device.
\end{itemize}
        
%
% Introduce the new possible approach (task-space synergies) and why it could be useful: human UL trajectory planning in task-space, able-bodied like motor behaviour.
%
\textbf{Introduce the new possible approach (task-space synergies) and why it could be useful}
\begin{itemize}
    \item Another possible synergy realisation, not yet considered in prosthetic interfaces, are task-space synergies \cite{Zeestraten2017}. In the prosthetic case, these relate the motion of the joints in the residual limb to a motion of the hand.
    \item These could have an advantage over joint-space synergies in terms of the resultant upper-limb motor behaviour (movement patterns), as it is theorised that upper-limb motion planning is done in task-space \cite{Uno1989, Wolpert1995, Flash2013, Kistemaker2014}.
    % How are these formulated in robotics
    \item From a robotics perspective, a task-space synergy can be generated using the manipulator's Jacobian \cite{Murray1994}. Assuming that knowledge of the initial conditions and the desired end-effector (hand) motion, then it is possible to find a relationship between the angular velocities of the joints in the arm.
    \item However, in the prosthetic case, knowing the desired hand motion before execution of the task is a challenge as this is only known to the human. While there are multiple approaches that attempt to solve this problem through additional information sources, this remains a challenge from a practical perspective.
    \item Regardless of the method used for the realisation of the synergistic prosthetic interface, their effects on motor behaviour are not widely understood due to the limited number of studies in the field to date.
\end{itemize}   

%
% Limitations of studies to date: lack of analysis of motor bevhaiour (movement patterns).
%
\textbf{Limitations of studies to date: lack of analysis of motor bevhaiour (movement patterns)}
\begin{itemize}
    \item Studies of synergistic prosthetic devices thus far have largely focused on evaluating performance of the task \cite{Kaliki2013, Blana2016, Alshammary2016}, with a few also evaluating their effects on the quantity of compensation motion \cite{Alshammary2018, Merad2016a, Merad2018}.
    \item Significant drive behind the study of synergies in transhumeral prostheses is based on the idea that these allow for natural motion. 
    \item Quality of motion and movement patterns are significant factors in assessing upper limb motor function and behaviour, and are typically used to evaluate recovery in rehabilitation environments \cite{Balasubramanian2012b, Balasubramanian2012, DeLosReyes-Guzman2014}. 
    \item However, some measures of quality of motion have only been considered as metrics for evaluating the effectiveness of a synergistic prosthetic elbow in \cite{Legrand2018}.
    \item Assessing the effects of synergistic prosthetic interfaces on motor behaviour, both in terms of quality of motion and movement patterns, is important in order to establish how these compare to able-bodied motion and whether they are effective at restoring natural motion.
\end{itemize}

%
% Contributions of this paper
%
\textbf{In this paper...}
\begin{itemize}
    \item This paper presents a study of quality of motion and movement patterns on able-bodied subjects using a virtual prosthetic elbow with different prosthetic interfaces in a Virtual Reality Environment.
    \item The objective of the study is to determine how synergistic prosthetic interfaces, both joint-space and task-space, perform in comparison to traditional prosthetic interfaces in terms of their capability to restore able-bodied motor behaviour.
    \item Given that task-space synergies are yet to be considered for transhumeral prosthetic applications, a novel method to realise these synergies in the context of the application is presented.
\end{itemize}

%
% Organisation
%
\textbf{Paper structure}
\begin{itemize}
    \item Prosposed method to realise task-space synergies in transhumeral prosthetics.
    \item Metrics used for the study of motor behaviour.
    \item Experimental methodology.
    \item Results.
    \item Discussion.
\end{itemize}

%
% Notation
%
The following notation is used throughout the paper. The set of real numbers is denoted as $\Real$, the set of positive real numbers is denoted as $\RealPos$. The left hand superscript $\frameOfRef{R}\xv$ is used to indicate the frame of reference $\{R\}$ of the vector $\xv$. The right hand superscript $x^{i}$ is used to indicate the iteration domain, such that $x^{i}$ indicates the $i$th iteration of $x$. $\| \cdot \|_2$ represents the Euclidean norm. %$\mu_t(\cdot)$ represents the mean over the time domain while $\mu_i(\cdot)$ represents the mean over the task iteration domain.

==> DotPointed/methodologyDP.tex <==
%
% Experimental methodology
%
\section{Experimental Methodology}
%
% Experiment objective
%
\begin{itemize}
    \item Experiment objective: To understand the effects of synergistic prosthetic interfaces on upper-limb motor behaviour, in terms of quality of motion and movement patterns, and determine the type of interface that produces the behaviour closest to natural able-bodied behaviour.
    \item The experiment was performed on able-bodied subjects in a Virtual Reality Environment (VRE) which was presented to the subjects with an HTC Vive Pro Head Mounted Display (HMD). This allowed to gather able-bodied motor behaviour data from subjects, and the virtually amputate and fit with a virtual prosthetic device in order to analyse motor behaviour with a prosthetic device.
    \item Focus of the experiment was on the use of the prosthetic device and how this use affects motion. As such, the prosthetic interface was simplified to reduce the cognitive burden of prosthesis use on subjects with no previous experience with such devices.
\end{itemize}

%
% Describe the experiment
%
\subsection{Experiment description}
%
% Present the task
%
\noindent \textbf{Present the task.}
\begin{itemize}
    \item The task required subjects to pick and place an object in 3D space in the forward direction from a standing position in a VRE.
    \item An iteration of the task is considered from when the object was grasped until the object was dropped off.
    \item Subjects were not allowed to step to perform the task.
    \item 1 object start position and 4 target positions.
\end{itemize}
%
% Present detail on the target locations.
%
\textbf{Present detail on the target locations.}
\begin{itemize}
    \item Start and target positions were normalised to each subject's height and arm length.
    \item The following reference frames were used:
    \begin{enumerate}
        \item Virtual world frame of reference. This frame of reference was chosen such that for the task the x-axis represents the forward direction, the y-axis the upwards direction, and the z-axis the lateral direction. The origin was placed on the floor under the position where the subjects were standing to perform the task.
        \item Sensor frame of reference. This frame of reference is determined by the sensor's yaw, pitch, and roll
    \end{enumerate}
    \item Let a subject's arm length be represented by $\ell$ and height by $h$. The target locations, in the virtual world frame of reference, are presented in Table \ref{ta:targets}.
    \begin{table}[ht]
    %\vspace{-3mm}
        \caption{Object start and target positions.}
        %\vspace{-2mm}
        \centering
        \begin{tabular}{|c||c|c|c|}
            \hline
            Target & $x (m)$ & $y (m)$ & $z (m)$  \\
            \hline
            \hline
            Start (ST)   &     $0.5\ell$     &     $0.5h$   &  0 \\
            \hline
            Close (CT)   &     $0.75\ell$    &     $0.65h$   &  0.12   \\
            \hline
            Mid (MT)   &     $1.0\ell$      &     $0.65h$   &  -0.12 \\
            \hline
            Far (FT)   &     $1.5\ell$      &     $0.65h$   &  0   \\
            \hline
            High (HT)   &     $1.0\ell$      &     $0.9h$   &  0   \\
            \hline
        \end{tabular}
        \label{ta:targets}
        %\vspace{-5mm}
    \end{table}
    
    The reasons for the choice of target locations were the following:
    \begin{itemize}
        \item Start (ST): Reachable from a neutral, relaxed position with the upper-arm down and elbow $90\deg$.
        \item Close (CT): A target that did not require the subject to use the prosthesis to perform the task.
        \item Mid (MT): A target that could be reached through either only using arm extension or compensation motion.
        \item Far (FT): A target that required both arm extension and upper-body lean to be reached.
        \item High (HT): A target that required both arm extension and shoulder motion to be reached.
    \end{itemize}
    These targets allow to study different movement patterns that occur on day-to-day reaching tasks in unstructured environments.
    \item An example for start and target positions for a subject in VRE are presented in Figure \ref{fig:sideView} and \ref{fig:subjectView}.
\end{itemize}
%
% Present detail on the modalities tested.
%
\textbf{Present detail on the modalities tested.}
\begin{itemize}  
    \item 4 different prosthetic interface modalities were considered for the experiment, 1 able-bodied and 3 transhumeral prosthetic:
    \begin{itemize}
        \item Able-bodied (AB). Used as the baseline for subject performance.
        \item sEMG proportional (EP). Most widely used interface modality for active prostheses. Dual-site differential sEMG activation commands the prosthetic elbow joint speed \cite{Fougner2012}.
        \item Joint-space kinematic synergy (JS). Most basic type of synergistic interface. Shoulder-elbow flexion synergy as given by $\dot{q}_e = \theta \dot{q}_s$ where $\dot{q}_s$ is the prosthetic elbow velocity, $\dot{q}_s$
        \item Task-space kinematic synergy (TS). The proposed task-space synergy method, where the synergy given by (\ref{eq:taskSpaceSynergy}).
    \end{itemize}
    \item The following prosthetic interface simplifications where done in order to reduce the cognitive load on the subjects and be able to focus the experiment on the motor behaviour aspect of prosthetic use:
    \begin{itemize}
        \item The functionality of the prosthetic elbow was enabled with a button press, instead of relying on complex sEMG switching commands, such as co-contraction, which are common place in prosthetics and are a major issue with active prosthetics to date \cite{Biddiss2007a}.
        \item Grasping and releasing of the object were done automatically when the subject stopped moving the hand and was touching the object (grasp) and within the target area (release). This avoided the need to switch between elbow and hand control.
    \end{itemize}
\end{itemize}

%
% Experiment set-up Figure
%
\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/TaskPOVAnnotated.png}
    \caption{Side view of the task. The object start position and target locations were normalised to the subject's height and arm length.}
    \label{fig:sideView}
\end{subfigure}
~
\begin{subfigure}[t]{0.315\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectPOVAnnotated.png}
    \caption{Subject point of view of the task. Only one target location was presented per repetition of the task and was selected randomly. Subjects were required to place the virtual hand on the orange circle before each repetition of the task.}
    \label{fig:subjectView}
\end{subfigure}

  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/AbleAvatarAnnotated.png}
    \caption{Able-bodied VR avatar. The forearm and hand motion trackers were used to create a forearm and hand avatar for the subject while the rest of the trackers were presented only as white markers. In the able bodied case, the elbow immobiliser was inactive to allow the subject to perform the task naturally. Grasping and dropping-off of the object were performed automatically.}
    \label{fig:ableAvatar}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/ProstheticAvatarAnnotated.png}
    \caption{Prosthetic VR avatar. The upper arm motion tracker was used to create a ``residual limb'' avatar to which the virtual prosthesis was attached while the rest of the trackers were presented only as white markers. In the prosthetic cases, the elbow immobiliser was engaged and forearm and hand tracking was disabled. Grasping and dropping-off of the object were performed automatically.}
    \label{fig:prosthesisAvatar}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectAnnotated.png}
    \caption{Subject with motion tracking sensors, elbow brace, and VR headset. Motion trackering sensors are highlighted by the yellow circles. Motion tracking sensors were placed on: C7 vertebrae, shoulder acromion, upper arm, forearm, and hand. An elbow immobiliser was used for the virtual prosthetic cases to better emulate prosthesis use. In the EMG case, two sEMG sensors were placed on the subject's forearm.}
    \label{fig:subject}
\end{subfigure} 
\caption{Experimental platform and task set-up.}
\label{fig:taskSetup}
\end{figure*}
%
% Figure END
%

%
% Describe the protocol
%
\subsection{Experiment protocol}
\begin{itemize}
    \item The experiment was performed on 15 able-bodied subjects, 6 female and 9 male.
    \item The age range was $[22, 34]$ and the median age $28$ years old.
    \item The experiment was performed in 2 different sessions lasting 2 hours each. Each session was done on different days, not more than a week apart. 
    \item Each session tested two different modalities. The first modality tested for all subjects was AB which was used as the baseline motor behaviour. The following modalities (prosthetic) were randomly selected to minimise the bias introduced by the effects of learning on the data gathered. The sessions procedure is presented in Table \ref{ta:protocol}.
    \begin{table}[ht]
    %\vspace{-3mm}
        \caption{Experiment session protocol.}
        %\vspace{-2mm}
        \centering
        \begin{tabular}{|c||c|c|}
            \hline
            Step & Time (minutes) & VR/No-VR \\
            \hline
            \hline
            Introduction   &     5     &     No-VR \\
            \hline
            Sensor placement   &     15   &     No-VR    \\
            \hline
            Modality 1  &     50      &     VR  \\
            \hline
            Break   &     5      &     No-VR  \\
            \hline
            Modality 2  &     50      &     VR  \\
            \hline
        \end{tabular}
        \label{ta:protocol}
        %\vspace{-5mm}
    \end{table}
    \item Each block for Modality testing consisted of 120 iterations of the task separated in 3 sets of 40 iterations. The procedure for each modality testing is presented in Table \ref{ta:modalityProtocol}.
    \begin{table}[ht]
    %\vspace{-3mm}
        \caption{Modality testing block protocol.}
        %\vspace{-2mm}
        \centering
        \begin{tabular}{|c||c|c|c|}
            \hline
            Step & Task iterations per target & Time (minutes) & VR/No-VR \\
            \hline
            \hline
            Training   &     -    &     5    &     No-VR \\
            \hline
            Practice   &     5    &     -    &     VR    \\
            \hline
            Set 1      &     10   &     -   &     VR  \\
            \hline
            Break   &     -      &     1    &     VR  \\
            \hline
            Set 2      &     10   &     -   &     VR  \\
            \hline
            Break   &     -      &     1    &     VR  \\
            \hline
            Set 3      &     10   &     -   &     VR  \\
            \hline
        \end{tabular}
        \label{ta:modalityProtocol}
        %\vspace{-5mm}
    \end{table}
    \item Only the last set of 40 iterations for each modality was used for data analysis in order to reduce the effects of motor learning on the results.
    \item Subjects were asked to use the prosthetic device as much as possible during the trials as the objective of the experiment was to analyse motor behaviour when the prosthetic device is used.
    \item Transhumeral amputation was emulated in able-bodied subjects in the VRE by using a motion sensor on the upper arm (Figure \ref{fig:subject}) which determined the motion of the virtual residual limb. A virtual prosthetic elbow, forearm, and hand were attached to the virtual residual limb. Further details on sensor placement and data gathering are presented in Section \ref{sec:dataGathering}.
    \item Figures \ref{fig:ableAvatar} and \ref{fig:prosthesisAvatar} show the VRE avatars for the able-bodied and prosthetic cases.
    \item During the Training block of the experiment subjects were instructed outside the VRE on how to use the prosthetic interface and were allowed to familiarise themselves with it. This was done by presenting a third person view of the virtual residual limb and prosthetic device on a screen.
\end{itemize}
The procedure was approved by the University of Melbourne Human Research Ethics Committee, project number 1750711.1. Informed consent was received from all subjects in the study. \textbf{ADD VIDEO OF EXPERIMENT}.

%
% Describe the protocol
%
\subsection{Data gathering}
\label{sec:dataGathering}
\begin{itemize}
    \item Upper-body, arm, and hand position and orientation in 3D space was gathered using motion trackers.
    \item Muscle activation, used for the EP modality, was gather using surface EMG electrodes.
    \item A summary of sensor type, location, and modalities where they were used are presented in Table \ref{ta:sensorInfo}.
    \item sEMG electrodes were placed on the forearm as the elbow brace interfered with the biceps/triceps eletrode placement used by transhumeral amputees. Furthermore, it was found that able-bodied subject had a difficulty to isolate biceps and triceps activation, which is required for the effective use of the EP modality.
    \item While this electrode position does not reflect the physiological placement of sEMG sensors for transhumeral prostheses, it provided comparable functional capabilities.
\end{itemize}
%
% Sensor placement table
%
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Sensor placement and information.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Location & Sensor type & Reference frame & Modalities \\
        \hline
        \hline
        C7 Vertebra &  Motion  & Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Shoulder &  Motion  &  Virtual world (position)  &  All \\
        acromion &          & Sensor (orientation)      & \\
        \hline
        Upper-arm &  Motion &  Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Lower-arm &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Hand    &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Forearm   &  sEMG &  -  &  EP \\
                  &       &     & \\
        \hline
    \end{tabular}
    \label{ta:sensorInfo}
    %\vspace{-5mm}
\end{table}


\subsection{Hardware set-up}
The experiment was performed on an HTC Vive Pro HMD with the application developed in Unity3D. The experimental platform runs on an Intel Core i7-8700K processor at 3.7GHz, with 32GB RAM, and an Gigabyte GeForce GTX 1080Ti video card with 11GB GDDR5. HTC Vive Trackers were used for motion tracking, except for hand motion tracking where a HTC Vive Controller was used (an analysis of HTC Vive system tracking capabilities can be found in \cite{Niehorster2017}). The Vive Trackers were attached directly to the subject's body using medical tape. Data gathering, and VR update were performed at 90Hz. Myoware sensors were used for sEMG data gathering with Ag-AgCl electrodes. The application used for the experiment can be downloaded from \textbf{ADD GITHUB LINK}.

==> DotPointed/metricsDP.tex <==
%
% Metrics for evaluating motor behaviour and performance
%
\section{Metrics for Evaluating Motor Behaviour and Performance}
Three categories of metrics are used in this paper to evaluate the effects of prosthetic interfaces on the following aspects of reaching motion: task performance, quality of motion, and motor behaviour.
%
% Task
%
\subsection{Task performance metrics}
\subsubsection{Task completion time ($t_f^{\mu}$)}
This metric is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature. The mean task time ($t_f^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:taskTime}
    t_f^{\mu} = \sum_{i=1}^{I}\frac{t_f^i}{I},
\end{equation}
where $t_f^i$ is the task end time for a given iteration $i$ and $I\subset\RealPos$ is the total number of iterations.
\subsubsection{Accuracy ($\delta^{\mu}$)}
This metric is used to verify that the task is being performed adequately. Let the desired hand target position be given by $\bar{\pv}_f$. Then the mean accuracy ($\delta^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:accuracy}
    \delta^{\mu} = \sum_{i=1}^{I}\frac{\|\bar{\pv}_f - \pv_f^i\|_2}{I},
\end{equation}
where $\pv_f^i$ is the hand final position for a given iteration $i$.

%
% Quality of motion
%
\subsection{Quality of motion metrics}
Two metrics for quality of motion are considered in this paper: path smoothness and variability.
\subsubsection{Path smoothness ($\eta$)}
\begin{itemize}
    \item Continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL) is used as the metric for smoothness \cite{Balasubramanian2012a} due to its characteristics which include sensitivity to changes in motor characteristics, robustness to measurement noise, provides a monotonic response (increase in movement complexity, increase in SAL), and is dimensionless.
\end{itemize}

Let $\xvd(t)$ be the hand ($\pvd(t)$) or joints ($\qvd(t)$) speed vector, such that the speed profile of the hand or joints is given by $v(t) = \| \xvd(t) \|_2$. $V(\omega)$ is the Fourier magnitude spectrum of $v(t)$, where $\omega\in \begin{bmatrix} 0,\omega_c \end{bmatrix}$ and $\omega_c = 40 rad/s$ which corresponds to the frequency range of motion of the human arm. Then, the spectral arc length of the path $\eta$ is given by \cite{Balasubramanian2012a}:
\begin{subequations}
\label{eq:smoothness}
\begin{align}
    \hat{V}(\omega) &= \frac{V(\omega)}{V(0)}, \\
    \eta &= -\int_{0}^{\omega_c} \sqrt{ \begin{pmatrix}
    \frac{1}{\omega_c}
    \end{pmatrix}^2 + \begin{pmatrix}
    \frac{ \partial\hat{V}(\omega) }{ \partial\omega }
    \end{pmatrix}^2} d\omega.
\end{align}
\end{subequations}
    
\subsubsection{Path variability ($\sigma_{\mu}$)}
\begin{itemize}
    \item Low path variability is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint) is considered as the metric for path variability.
\end{itemize}

The hand/joint path variability metric ($\sigma_{\mu}$) is defined herein by the mean standard deviation of the hand/joint path across the time domain as follows. Let the hand or joint path vector for a given iteration $i$ be $\xv^i(t_s n)$ and the mean path vector over the $I$ number of iterations be $\xv^{\mu}(t_s n)$. $t_s > 0$ is the path sampling time and $n\in N$ the sample number, where $N\subset\RealPos$. 
\begin{subequations}
\label{eq:handSTD}
\begin{align}
    \sigmav(t_s n) &= \sqrt{ \frac{\sum_{i=1}^{I}(\xv^i(t_s n)   - \xv^{\mu}(t_s n) )^2 }{I} }, \\
    \sigma_{\mu} &= \sum_{n=0}^{N}\frac{\sigmav(t_s n)}{N}.
\end{align}
\end{subequations}

%
% Motor behaviour
%
\subsection{Motor behaviour metrics}
\begin{itemize}
    \item Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion.
    \item The metrics used in this paper use individual able-bodied motion as the point of reference for each subject.
    \item To provide a deeper analysis of motor behaviour, particularly with respect to movement patters, individual behaviour will also be analysed in the results section in addition to the metrics presented next.
\end{itemize}
\subsubsection{Path difference ($\Delta_{\mu}$)}
This metric evaluates the difference between the mean able-bodied hand or joint path and the mean prosthetic hand or joint path. This is used to determine the closeness of the resultant prosthetic motor behaviour to the individual's natural able-bodied motor behaviour. Let the mean hand or joint path for the able-bodied case ($AB$) be given by $\xv_{AB}^{\mu}(t_s n)$ and the mean path for the prosthetic case ($PC$) given by $\xv_{PC}^{\mu}(t_s n)$. The path difference ($\Delta_{\mu}$) is defined as the mean absolute difference between the mean paths across the time domain as follows.

\begin{subequations}
\label{eq:handDiff}
\begin{align}
    \Deltav(t_s n) &=  \left | \xv_{AB}^{\mu}(t_s n)- \xv_{PC}^{\mu}(t_s n) \right |, \\
    \Delta_{\mu} &=  \sum_{n=0}^{N}\frac{\| \Deltav_p(t_s n) \|_2}{N}.
\end{align}
\end{subequations}

\subsubsection{Upper-body displacement ($\phi^{\mu}$)}
This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Some level of upper-body motion is also part of natural able-bodied motion during reaching tasks. Let the position of the part of the upper-body to be analysed be given by $\pv_{UB}(t)\in\Real^3$. The metric is defined as follows:
\begin{subequations}
\label{eq:motionMagnitude}
\begin{align}
    \phiv^i &=  \| \pv_{UB}^i(t_f) - \pv_{UB}^i(0)\|_2, \\
    \phi^{\mu} &=  \sum_{i=1}^{I}\frac{\phiv^i }{I}.
\end{align}
\end{subequations}


==> DotPointed/resultsDP.tex <==
%
% Experiment results
%
\section{Results}
\begin{itemize}
    \item Hand paths for all modalities and targets were normalised to the subject's arm length for their analysis similarly to \cite{Yang2002}.
    \item The data-set can be downloaded from \textbf{ADD GITHUB LINK}.
\end{itemize}
%
% Task
%
\subsection{Task performance metrics}

%
% Time
%
\subsubsection{Task completion time ($t_f^{\mu}$)}
\begin{itemize}
    \item Results for task completion time are presented in Figure \ref{fig:time}, where the mean task completion time for the experiment population is presented for each modality and target.
    \item Synergistic interfaces were 20\% faster than sEMG for the Far target.
    \item Synergistic interfaces (TS, JS) show an advantage in task completion time over EP for the Far target, which requires the more complex coordinated motion (upper-body and upper-arm).
    \item This suggests that when EP can be used effectively and there is no sequential switching between the joints in the limb it can be as effective as synergistic interfaces.
    \item \cite{Alshammary2018} showed that there was a significant reduction in task completion time with JS assisted EP; however, the study could not identify whether this was due to the motion activated elbow/hand sEMG switching or the synergistic interface itself. The results presented herein along with those presented in \cite{Alshammary2018} suggest that synergistic interfaces may prove to be most effective in multi-degree of freedom prostheses and complex tasks.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/01_TaskTime.eps}
    \caption{Population task completion time mean and standard deviation.}
    \label{fig:time}
\end{figure}

%
% Accuracy
%
\subsubsection{Accuracy ($\delta^{\mu}$)}
\begin{itemize}
    \item Results for reach accuracy are presented in Figure \ref{fig:accuracy}, where the mean reach accuracy for the experiment population is presented for each modality and target.
    \item The results show that subjects were capable of performing the task with similar accuracy for all modalities and targets.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/02_Accuracy.eps}
    \caption{Population reach accuracy mean and standard deviation.}
    \label{fig:accuracy}
\end{figure}

%
% Quality of motion
%
\subsection{Quality of motion metrics}
%
% Hand smoothness
%
\subsubsection{Hand path smoothness ($\eta_v$)}
\begin{itemize}
    \item Results for hand smoothness are presented in Figure \ref{fig:handSAL}, where the mean hand path spectral arc length for the experiment population is presented for each modality and target.
    \item These results can be affected if the subject chose to not use, or to pre-position, the prosthetic device during an trial. This is because a movement that only includes the ``healthy'' joints of the subject will be inherently smooth.
    \item This effect can be clearly seen in the Close and High targets, as EP was rarely used as was unnecessary.
    \item The JS interface shows a 10\% improvement in smoothness for the Far target with respect to the EP and TS interfaces.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/03_HandSAL.eps}
    \caption{Population hand path smoothness mean and standard deviation. The less negative the smoother the path.}
    \label{fig:handSAL}
\end{figure}

%
% Joint smoothness
%
\subsubsection{Joint path smoothness ($\eta_q$)}
\begin{itemize}
    \item Results for joint smoothness are presented in Figure \ref{fig:jointSAL}, where the mean joints path spectral arc length for the experiment population is presented for each modality and target.
    \item In this instance the JS modality shows an improvement over the other prosthetic interfaces for the Mid, Far, and High targets. The joint motion was 18\%, 24\%, and 15\% smoother than EP for the Mid, Far, and High targets respectively.
    \item On the other hand, the TS modality only shows a 17\% improvement in joint smoothness for the Far target with respect to the EP.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/04_JointSAL.eps}
    \caption{Population joint path smoothness mean and standard deviation. The less negative the smoother the path.}
    \label{fig:jointSAL}
\end{figure}

%
% Hand path variation
%
\subsubsection{Standard deviation of the hand trajectory ($\sigma_{\mu, p}$)}
\begin{itemize}
    \item Results for hand path variability are presented in Figure \ref{fig:handVar}, where the mean hand path standard deviation for the experiment population is presented for each modality and target.
    \item The synergistic interfaces show lower hand path variability over EP for the Far target, with TS showing a 16\% reduction in variability over EP and JS a 31\% reduction.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/05_HandPathVar.eps}
    \caption{Population hand path variability mean and standard deviation.}
    \label{fig:handVar}
\end{figure}

%
% Joint path variation
%
\subsubsection{Standard deviation of the joint trajectory ($\sigma_{\mu, q}$)}
\begin{itemize}
    \item Results for joint path variability are presented in Figure \ref{fig:jointVar}, where the mean joint path standard deviation for the experiment population is presented for each modality and target.
    \item The synergistic interfaces show lower joint path variability over EP for the Far and High targets; however, EP and TS show high inter-subject variability for the High target.
    \item For the Far target case TS shows a 20\% reduction in joint path variability over EP while JS a 31\% reduction over EP.
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/05_2_JointPathVar.eps}
    \caption{Population joint path variability mean and standard deviation.}
    \label{fig:jointVar}
\end{figure}
%
% Motor behaviour
%
\subsection{Motor behaviour metrics}
%
% Hand path difference
%
\subsubsection{Hand path difference ($\Delta_{\mu, p}$)}
\begin{itemize}
    \item Results for hand path difference are presented in Figure \ref{fig:handDiff}, where the mean difference between the able-bodied hand path and the prosthetic modalities hand path for the experiment population is presented for each prosthetic modality and target.
    \item The JS modality shows an improvement over the other prosthetic interfaces for the Far target, being 24\% closer to the able-bodied hand path than EP and TS.
    \item This suggests that for complex coordinated movements the JS interface may be able to render the more natural hand path.
    \item Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}. 
\end{itemize}
%
% Figure
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/07_HandPathDifference.eps}
    \caption{Population hand path difference mean and standard deviation.}
    \label{fig:handDiff}
\end{figure}

%
% Joints relationship difference
%
\subsubsection{Joints relationship difference ($\Delta_{\mu, q}$)}
\begin{itemize}
    \item Results for joints relationship difference are presented in Figure \ref{fig:jointDiff}, where the mean difference between the able-bodied joints relationship and the prosthetic modalities hand path for the experiment population is presented for each prosthetic modality and target.
    \item The JS modality shows an improvement over the other prosthetic interfaces for the Close and Far targets. JS is 28\% closer to able-bodied joint behaviour than EP and TS for the Close target, and 19\% and 35\% closer than EP and TS to able-bodied joint behaviour for the Far target.
    \item The result for the Far target suggests that for complex coordinated movements the JS interface may be able to render the more natural hand path.
    \item It is important to note that there is a high degree of inter-subject variability for the EP modality while TS and JS show lower variability. This suggests that subjects were consistently capable of effectively using the synergistic interfaces, unlike with EP where some subjects may not have been able to use it effectively. This highlights the intuitiveness of synergistic interfaces, which suggests that they may be easier to learn.
    \item Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}.
\end{itemize}
%
% Figure
%
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/Results/08_JointPathDifference.eps}
    \caption{Population joint path difference mean and standard deviation.}
    \label{fig:jointDiff}
\end{figure}

%
% Upper-body displacement
%
\subsubsection{Upper-body displacement ($\phi_{\mu}$)}
\begin{itemize}
    \item Results for upper-body displacement are presented in Figure \ref{fig:UBDisplacement}, where the mean C7 and shoulder acromion displacement for the experiment population are presented in Figures \ref{fig:C7Displacement} and \ref{fig:SADisplacement}, respectively, for each modality and target.
    \item These results show that subjects performed the task with similar upper-body displacement across all modalities, meaning that they purposely used the prosthetic devices to perform the task as instructed. As such, the effects of prosthetic interfaces on motor behaviour in this study are better determined by the trajectories rather than the resultant upper-body displacement.
\end{itemize}
%
% Figure
\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/Results/06_1_C7Displacement.eps}
    \caption{Population C7 displacement mean and standard deviation.}
    \label{fig:C7Displacement}
\end{subfigure}

  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/Results/06_2_SADisplacement.eps}
    \caption{Population shoulder acromion displacement mean and standard deviation.}
    \label{fig:SADisplacement}
\end{subfigure}
\caption{Upper-body displacement results.}
\label{fig:UBDisplacement}
\end{figure}


%
% Motion patterns analysis
%
\subsection{Motion patterns analysis}
Given that the more significant motor behaviour changes are observed for the Far target, the motion patern analysis will focus on the results for such target.
\subsubsection{Hand path}
Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}. 
\begin{itemize}
    \item The normalised AB hand path follows the shape typically seen in reaching movements \cite{Yang2002}, this shows that the VRE did not affect the motor behaviour of subjects.
    \item While some subjects were not able of achieving able-bodied-like hand motion with any type of prosthetic interface within the time allowed for the experiment, some interesting patterns can be observed in these results.
    \item As expected from the EP case, the hand follows a more irregular path as the user manually adjusts the elbow position throughout the reaching motion.
    \item The two step movement strategy required by the TS interface can seen in the results for subjects 8, 12, 14. The strategy involves an initial hand pre-position movement characterised by a smooth upward/forward hand movement, followed by a mostly straight hand path due to the task-space synergy. While this behaviour was also observed in the task iteration results of the other subjects, these do not appear in the mean hand path due to averaging effects. 
    \item It should also be noted that subjects 3, 6, 11 were capable of achieving on average a TS hand path nearly identical to their AB. This suggests that these subjects found a way to utilise the interface to achieve the most natural hand path.
    \item On the other hand, a larger number of subjects were capable of achieving nearly overlapping AB hand path with the JS interface, subjects 2, 3, 5, 6, 10, 14. This suggests that JS may be easier to learn due to its reduced complexity. 
    \item These differences are captured by the metrics related to hand quality of motion and behaviour $\eta_v$, $\sigma_{\mu,p}$, and $\Delta_{\mu,p}$, where JS performed better than TS
\end{itemize}
%
% Figure
%
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Results/09_HandFunnels.eps}
    \caption{Mean hand path for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green.}
    \label{fig:handFunnels}
\end{figure*}


\subsubsection{Shoulder-elbow flexion relationship}
Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}. \textbf{NOTE: This is technically the average synergy!}
\begin{itemize}
    \item The AB shoulder-elbow relationship is characterised for being a smooth curve.
    \item EP is composed of two mostly straight lines, one horizontal and one vertical or with high slope. These correspond to mostly sequential shoulder and elbow motion. This behaviour is commonly seen with this type of prosthetic interface.
    \item TS is composed of a straight horizontal line and a smooth curve. These correspond to the initial pre-positioning of the hand followed by a coordinated movement. Given that the interface was designed to operate in such way due to the lack of information (target position), this resultant behaviour is expected. This highlights how the interface design can directly affect the motor behaviour of prosthesis users and should be taken in consideration when designing prosthetic interfaces.
    \item JS is composed of a smooth curve in most subjects, pointing towards a mostly coordinated movement. This is an interesting result as it suggests that the subjects learned to use the synergy enabling mechanism (button press) to activate the elbow such that the most natural reaching motion possible was performed.
    \item In some subjects, for both TS and JS, it is possible to observe a short shoulder only movement at the end of the reach (e.g. subject 4). This is appears as a result of having to compensate for an inaccurate initial reach, which then needed to be corrected while elbow was fixed in position as otherwise it would result in elbow flexion.
    \item These differences in motor behaviour between TS and JS are captured by the joint path smoothness ($\eta_{\mu,q}$) and difference metrics ($\Delta_{\mu,q}$), where JS performed better than TS.
\end{itemize}
%
% Figure
%
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Results/10_JointFunnels.eps}
    \caption{Mean shoulder-elbow flexion relationship for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green. The origin represents the arm extended forward.}
    \label{fig:jointFunnels}
\end{figure*}

==> Outlines/1_intro_outline.tex <==
%
% Introduction
%
\section{Introduction}
%
%
\begin{itemize}
%
% What is the main challenge that we are studying in this paper?
% Coordinated motion is required for ADLs.
% This is not possible with current prostheses.
%
    \item Coordinated arm motion is required for most Activities of Daily Living (ADLs).
    \item Current prosthetic devices are only capable of sequential Degree of Freedom (DOF) motion.
    
    
%
% What is a possible solution for this challenge in the literature?
% A novel kinematic synergy based HPI allows for coordinated motion.
%
    \item In the context of transhumeral prostheses, novel human-prosthetic interfaces, such as kinematic synergy and pattern recognition based interfaces \cite{Alshammary2018,Ortiz-Catalan2014}, permit the coordinated motion of multiple prosthesis DOFs with those of the residual limb.
    \item Kinematic synergies in human-prosthetic interfaces (referred to as HPIs henceforth) directly relate the motion of the residual limb with that of the prosthesis.
    
    
%
% What are the limitations of this solution?
% Synergies are individual and task/path dependent.
%
    \item The synergies in these interfaces have been observed to be individual and task/path dependent \cite{Merad2018, Gottlieb1997}.
    
%
% What are possible solutions to these limitations in the literature?
% Personalization, our work.
% Task dependency is still an open question. Examples of how the synergy depends on start and end position. How it is possible to reach in 3D from a single start point.
%
    \item Task/path dependency has not been fully addressed in the literature so far.
    \item Kinematic synergies for HPIs have been formulated in the literature as either dependent on residual limb joints angular position or velocity \cite{Legrand2018,Alshammary2018}.
    \item This type of formulation has been considered for specific starting positions with the ability to reach multiple targets \cite{Legrand2018, Akhtar2017, Blana2016}, where the obtained synergy depends on the starting position.
    \item However, ADLs and reaching tasks are variable in terms of the start and end positions.
    \item This formulation has also been shown to have the same result on able-bodied individuals \cite{Bockemuhl2010}.
    
%
% What do these lack?
% We know from traditional kinematic analysis that end effector path is a function of both the joints angular position and velocity. All current formulations only consider either one.
%
    \item From traditional kinematic analysis of mechanical systems, we know that the end effector path is a function of both the joints angular position and velocity \cite{Murray1994}.
%
% What is this paper about?
% Systematic formulation of synergistic motion in the context of upper limb prosthesis independent of initial and final arm posture.
% We propose a kinematic synergy HPI based on traditional robotics kinematic analysis, where the path of the hand is determined by a function of the joints angular position and velocity.
%
    \item In this paper:
    \begin{itemize}
        \item Systematic formulation of synergistic motion in the context of upper limb prosthesis independent of initial and final arm posture.
        \item We propose a kinematic synergy HPI based on traditional kinematic analysis, where the velocity profile of the hand is determined by the arm Jacobian, a function of the joints angular position and velocity.
    \end{itemize}
%
\end{itemize}


%
% Notation
%
The following notation is used throughout the paper. The set of real numbers is denoted as $\Real$, the set of positive real numbers is denoted as $\RealPos$. The left hand superscript $\frameOfRef{R}x$ is used to indicate the frame of reference. The right hand superscript $x^{i}$ is used to indicate the iteration domain, such that $x^{i}$ indicates the $i$th iteration of $x$.

==> Outlines/2_formulation_outline.tex <==
%
% Problem formulation
%
\section{Problem formulation}
%
% Formulate in problem in terms of the kinematic analysis
%
\begin{itemize}
    \item General reaching tasks can have infinite possibilities in terms of their start and end position, making it difficult to determine a general case synergy to account for all motion.
    \item From the kinematic analysis of the arm, the following relationship between hand path velocity and joint angular velocities is known
    \begin{equation}
        \vv = \Jacob(\qv_s,\qv_e)\begin{bmatrix} \qvd_s & \qvd_e \end{bmatrix}^T,
    \end{equation}
    where $\vv\in\Real^3$ is the hand velocity in task space. $\qv_s$ and $\qvd_s$ represent residual limb joint angular displacement and velocity respectively, for the transhumeral amputation case $\qv_s\in\Real^3$ and $\qvd_s\in\Real^3$. $\qv_e$ and $\qvd_e$ represent prosthesis joint angular displacement and velocity respectively. $\mcl{J}(\qv_s,\qv_e)$ is the arm Jacobian.
    \item For the elbow prosthesis case $\qv_s\in\Real$ and $\qvd_s\in\Real$. 
    \item Assuming that knowledge of the initial conditions and the desired hand motion ($\vv$), it is possible to find a relationship between the residual limb joints and the prosthesis joints angular velocities, $\qvd_s$ and $\qvd_e$ respectively.
    \item However, in the prosthetic case, knowing the desired hand motion ($\vv$) before execution of the task is a challenge as this is only known to the human.
    
    \item 
    \item In order to simplify the problem, we can take inspiration from the synergistic motion analysis literature, where it has been reported that:
    \begin{itemize}
        \item Reaching motion can be normalized such that the hand path is invariant of the start and end positions \cite{Yang2002}.
        \item Forward reaching motion has been found to be most significantly related to the synergy between shoulder and elbow flexion/extension \cite{Bockemuhl2010}.
    \end{itemize}
    
    \item
    \item We constrain the problem to forward reaching motion, as there is a clear relationship of the synergies involved.
    \item This restricts the admissible path to a subset of the full range of able-bodied arm motion, which is a trade-off between practical functionality and generality of the approach.
    \item Figure \ref{fig:reaching1} presents an example of a target reaching task. By first re-positioning the hand to be aligned with the target on a forward reaching path, the required knowledge of the task can be diminished.
    \item With this, it is possible to constrain the desired hand path such that it behaves as sliding on a forward path.
    \item Figure \ref{fig:reaching2} presents the proposed simplified geometry to be used to define the desired hand path.
\end{itemize}

    \begin{figure*}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching1.png}
        \caption{Target reaching example. The green dotted line shows the shortest path to target. The orange dotted line the forward straight reaching path. The reference frame represented by the subscript $r$ has its origin at the shoulder with the $x$-axis pointing forward.}
        \label{fig:reaching1}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching2.png}
        \caption{Simplified geometry for a reaching task by re-positioning the hand. The hand slides across the forward reaching path. The $x_s$-$z_s$ plane is parallel to the ground.}
        \label{fig:reaching2}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching3.png}
        \caption{Definition of the motion direction ($d$) and hand ($h$) frames that determine the forward reaching motion. The direction frame is defined by the triangle created by the shoulder (S), elbow (E), and hand (H) joints and it has its origin at the shoulder joint.}
        \label{fig:reaching3}
    \end{subfigure}
    \caption{Formulation of the forward reaching task and reference motion for the Jacobian-based synergistic prosthesis interface.}
    \label{fig:reaching}
    \end{figure*}
    
\subsection{Jacobian-based kinematic synergy formulation}
\begin{itemize}
    \item 
    \item In order to obtain the synergy between the shoulder and elbow the following steps are followed:
    \begin{itemize}
        \item For a given task start position.
        \item Determine the direction of motion reference frame ($D$).
        \item Determine shoulder and elbow joint angular displacement with reference to $D$.
        \item Determine the arm Jacobian and the hand motion constraint on $\frameOfRef{D}x_h$.
        \item Solve for $\qvd_e$ to determine the synergy.
    \end{itemize}
    \item \textbf{Assumptions:}
    \begin{itemize}
        \item The angular position and velocities of the residual limb are measurable. 
        Remark: IMU-based measurements of residual limb motion have been demonstrated for synergistic elbow prostheses in \cite{Merad2016a}.
        \item The physical properties of the human-prosthesis arm, such as joint-to-joint distance, are known.
    \end{itemize}
    \item Direction of motion reference frame:
    \begin{itemize}
        \item Let the origin of the direction of motion frame ($D$) be located at the shoulder joint center. The direction frame w.r.t. the reference frame is defined as follows:
        \begin{itemize}
            \item $x_d$-axis: given in the direction from the shoulder joint center to the initial hand position $\pv$.
            \begin{equation}
                \frameOfRef{R}x_d = \frac{\frameOfRef{R}\pv}{\|\frameOfRef{R}\pv\|}
            \end{equation}
            \item $z_d$-axis: perpendicular to the plane given by the S-E-H triangle, in the direction of $z_r$. This can be defined by
            \begin{equation}
                \frameOfRef{R}z_d =  \frac{ \frameOfRef{R}r_{RE} \times \frameOfRef{R}x_d }{\|\frameOfRef{R}r_{RE} \times \frameOfRef{R}x_d\|}
            \end{equation}
            where $\frameOfRef{R}r_{RE}$ is the vector from the shoulder to the elbow joint.
            \item $y_d$-axis: follows the right hand rule.
        \end{itemize}
        \item With this the direction of motion reference frame ($D$) is defined and motion of the arm and hand can be expressed with it as reference.
    \end{itemize}
    \item
    \item Arm Jacobian:
    \begin{itemize}
        \item By considering the forward reaching task on the direction of motion frame, the task is simplified to a basic 2-DOF planar arm.
        \item The differential kinematics of the simplified arm are given by:
        \begin{subequations}
        \label{eq:simpDiffKine}
        \begin{align}
            \bar{\vv} &= \bar{\Jacob}(\bar{q}_s,\bar{q}_e)\begin{bmatrix} \dot{q}_s & \dot{q}_e \end{bmatrix}^T,\\
            \bar{\Jacob}(\bar{q}_s,\bar{q}_e) &= \begin{bmatrix}
            -\ell_{u} S_s - \ell_{l} S_{se} & -\ell_{l} S_{se}\\
            \ell_{u} C_s + \ell_{l} C_{se} & \ell_{l} C_{se}
            \end{bmatrix}.
        \end{align}
        \end{subequations}
        where $C_s = \cos{(\bar{q}_{s})}$, $S_s = \sin{(\bar{q}_{s})}$, $C_{se} = \cos{(\bar{q}_{s} + \bar{q}_{e})}$, $S_{se} = \sin{(\bar{q}_{s} + \bar{q}_{e})}$, $\bar{q}_{s} = \frameOfRef{D}q_{s}$, $\bar{q}_{e} = \frameOfRef{D}q_{e}$, and $\bar{\vv} = \begin{bmatrix} ^{D}\dot{x} & ^{D}\dot{y} \end{bmatrix}^T$.
    \end{itemize}
    \item
    \item Shoulder-elbow synergy:
    \begin{itemize}
        \item As previously discussed, only the forward reaching motion is required along the direction of motion plane. This means that it is desired to satisfy the constraint $^{D}\dot{y} = 0$.
        \item With this it is possible to solve from Equation (\ref{eq:simpDiffKine}) for the desired elbow velocity $\dot{q}_e$, such that
        \begin{equation}
            \dot{q}_e = -\ell_{l} C^{-1}_{se}(\ell_{u} C_s + \ell_{l} C_{se})\dot{q}_s.
        \end{equation}
        \item Remark: it is important to note that a singularity exists when $\bar{q}_{s} + \bar{q}_{e} = n\pi/2$, $n = 1, 2, \cdots$; and needs to be properly handled.
    \end{itemize}
\end{itemize}

==> Outlines/4_metrics_outline.tex <==
%
% Metrics for evaluating motor behaviour and performance
%
\section{Metrics for Evaluating Motor Behaviour and Performance}

%
% Task
%
\subsection{Task performance metrics}
\subsubsection{Task completion time ($t_f^{\mu}$)}
This metric is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature. The mean task time ($t_f^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:taskTime}
    t_f^{\mu} = \sum_{i=1}^{I}\frac{t_f^i}{I},
\end{equation}
where $t_f^i$ is the task end time for a given iteration $i$ and $I\in\RealPos$ is the total number of iterations.
\subsubsection{Accuracy ($\delta^{\mu}$)}
This metric is used to verify that the task is being performed adequately. Let the desired hand target position be given by $\bar{\pv}_f$. Then the mean accuracy ($\delta^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:accuracy}
    \delta^{\mu} = \sum_{i=1}^{I}\frac{\|\bar{\pv}_f - \pv_f^i\|_2}{I},
\end{equation}
where $\pv_f^i$ is the hand final position for a given iteration $i$.

%
% Quality of motion
%
\subsection{Quality of motion metrics}
Two metrics for quality of motion are considered in this paper:
\begin{itemize}
    \item \textbf{Smoothness:} continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL) is used as the metric for smoothness \cite{Balasubramanian2012a}.
    \begin{itemize}
        \item A healthy, trained upper-limb reaching movement, considered smooth, is usually composed of a single low frequency component. This type of movement results in simple Fourier magnitude spectrum.
        \item On the other hand, non-natural movement which tend to be jerky, considered non-smooth, are usually composed of a main low frequency main movement, along with high frequency undesirable movements. This type of movement results in a complex Fourier magnitude spectrum.
        \item Example figure with resultant SAL for both cases: hand path, Fourier magnitude spectrum, SAL.
        \item Spectral arc length measures the complexity of the Fourier magnitude spectrum of the velocity profile through the arc length of such spectrum.
        \item This metric has the following advantages: sensitive to changes in motor characteristics, robust to measurement noise, monotonic response (increase in complexity, increase in SAL), and dimensionless.
    \end{itemize}
\end{itemize}
\subsubsection{Hand path smoothness ($\eta_v$)}
Let $v(t) = \| \vv(t) \|_2$ be the speed profile of the hand and $V(\omega)$ its Fourier magnitude spectrum, where $\omega\in \begin{bmatrix} 0,\omega_c \end{bmatrix}$ and $\omega_c = 40 rad/s$ which corresponds to the frequency range of motion of the human arm. Then, the spectral arc length of the hand path $\eta_v$ is given by \cite{Balasubramanian2012a}:
\begin{subequations}
\label{eq:handSmoothness}
\begin{align}
    \hat{V}(\omega) &= \frac{V(\omega)}{V(0)}, \\
    \eta_v &= -\int_{0}^{\omega_c} \sqrt{ \begin{pmatrix}
    \frac{1}{\omega_c}
    \end{pmatrix}^2 + \begin{pmatrix}
    \frac{ \partial\hat{V}(\omega) }{ \partial\omega }
    \end{pmatrix}^2} d\omega.
\end{align}
\end{subequations}

\subsubsection{Joint path smoothness ($\eta_q$)}
Let $\dot{q}(t) = \| \qvd(t) \|_2$ be the speed profile of the upper-limb joint-space and $Q(\omega)$ its Fourier magnitude spectrum, where $\omega\in \begin{bmatrix} 0,\omega_c \end{bmatrix}$ and $\omega_c = 40 rad/s$ which corresponds to the frequency range of motion of the human arm. Then, the spectral arc length of the joint path $\eta_q$ is given by \cite{Balasubramanian2012a}:
\begin{subequations}
\label{eq:jointSmoothness}
\begin{align}
    \hat{Q}(\omega) &= \frac{Q(\omega)}{Q(0)}, \\
    \eta_q &= -\int_{0}^{\omega_c} \sqrt{ \begin{pmatrix}
    \frac{1}{\omega_c}
    \end{pmatrix}^2 + \begin{pmatrix}
    \frac{ \partial\hat{Q}(\omega) }{ \partial\omega }
    \end{pmatrix}^2} d\omega.
\end{align}
\end{subequations}
    
\begin{itemize}
    \item \textbf{Path variability:} low path variability is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint) is considered as the metric for path variability.
\end{itemize}

\subsubsection{Standard deviation of the hand trajectory ($\sigma_{\mu p}$)}
\begin{subequations}
\label{eq:handSTD}
\begin{align}
    \sigmav_p(t) &= \sqrt{ \frac{\sum_{i=0}^n(\pv^i(t)   - \pv^{\mu}(t) )^2 }{n} }, \\
    \sigma_{\mu p} &= \mu_t (\| \sigmav_p(t) \|_2).
\end{align}
\end{subequations}
Where $i$ represents an iterations of the task, $n$ the total number of iterations of the task, and $\pv^{\mu}(t)$ is the mean hand path for the given task. Then $\sigma_{\mu p}$ is the mean standard deviation of the hand trajectory across the time domain.
\subsubsection{Standard deviation of the joint trajectory ($\sigma_{\mu q}$)}
\begin{subequations}
\label{eq:jointSTD}
\begin{align}
    \sigmav_q(t) &= \sqrt{ \frac{\sum_{i = 1}^n(\qv^i(t)  - \qv^{\mu}(t))^2 }{n} }, \\
    \sigma_{\mu q} &= \mu_t (\| \sigmav_q(t) \|_2).
\end{align}
\end{subequations}
Where $i$ represents an iterations of the task, $n$ the total number of iterations of the task, and $\qv^{\mu}(t)$ is the mean joint path for the given task. Then $\sigma_{\mu q}$ is the mean standard deviation of the joint trajectory across the time domain.

%
% Motor behaviour
%
\subsection{Motor behaviour metrics}
\begin{itemize}
    \item Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion.
    \item The metrics used in this paper use individual able-bodied motion as the point of reference for each subject.
    \item To provide a deeper analysis of motor behaviour, particularly with respect to movement patters, individual behaviour will also be analysed in the results section in addition to the metrics presented next.
\end{itemize}
\subsubsection{Hand path difference ($\Delta_{\mu p}$)}
This metric evaluates the difference between the mean able-bodied hand path and the mean prosthetic hand path. This is used to determine the closeness of the resultant prosthetic motor behaviour, in task-space, to the individual's natural able-bodied motor behaviour. The hand path difference is calculated as:

\begin{subequations}
\label{eq:handDiff}
\begin{align}
    \Deltav_p(t) &=  \left | \pv_{AB}^{\mu}(t)- \pv_{PC}^{\mu}(t) \right |, \\
    \Delta_{\mu p} &=  \mu_t( \| \Deltav_p(t) \|_2).
\end{align}
\end{subequations}
$\pv_{AB}^{\mu}(t)$ is the mean hand path for the given task for the able-bodied case. $\pv_{PC}^{\mu}(t)$ is the mean hand path for the given task for a prosthetic case (EP, TS, JS). Then $\Delta_{\mu p}$ is the mean difference of the mean hand trajectories across the time domain.

\subsubsection{Joints relationship difference ($\Delta_{\mu q}$)}
This metric evaluates the difference between the mean able-bodied joints relationship and the mean prosthetic joints relationship. This is used to determine the closeness of the resultant prosthetic motor behaviour, in joint-space, to the individual's natural able-bodied motor behaviour. The joint path difference is calculated as:

\begin{subequations}
\label{eq:jointDiff}
\begin{align}
    \Deltav_q(t) &=  \left | \qv_{AB}^{\mu}(t)- \qv_{PC}^{\mu}(t) \right |, \\
    \Delta_{\mu q} &=  \mu_t( \| \Deltav_q(t) \|_2).
\end{align}
\end{subequations}
$\qv_{AB}^{\mu}(t)$ is the mean joints path for the given task for the able-bodied case. $\qv_{PC}^{\mu}(t)$ is the mean joints path for the given task for a prosthetic case (EP, TS, JS). Then $\Delta_{\mu q}$ is the mean difference of the mean hand trajectories across the time domain.

\subsubsection{Upper-body displacement ($\phi_{\mu ub}$)}
This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Upper-body motion is also part of natural able-bodied motion during reaching tasks. Let the position of the part of the upper-body to be analysed be given by $\pv_{UB}(t)\in\Real^3$. The metric is defined as follows:
\begin{subequations}
\label{eq:motionMagnitude}
\begin{align}
    \phiv_{ub}(i) &=  \pv_{UB}^i(t_f) - \pv_{UB}^i(0), \\
    \phi_{\mu ub} &=  \mu_i( \| \phiv_{ub}(i) \|_2).
\end{align}
\end{subequations}


==> old/1_intro_vBM.tex <==
%
% Introduction
%
\section{Introduction}
%
%

%
% Introduce synergies in prosthetics and their advantages.
%

Synergistic prosthetic interfaces in upper-limb prostheses enable the coordinated human-prosthetic arm motion required by many activities of daily living. Motion-based synergistic interfaces determine the motion of the prosthetic device as a function of the motion the residual limb \cite{Akhtar2017}, thus allowing complex coordinated motion that is otherwise not possible with traditional surface electromyography (sEMG) based interfaces.
%
% Describe the current method used to realise synergies in transhumeral prosthetics: joint-space synergies
The typical realisation of synergies in prosthetic interfaces are joint-space synergies \cite{Akhtar2017, Kaliki2013, Blana2016, Legrand2018, Alshammary2018, Garcia-Rosas2019}. These relate the motion of the joints in the residual limb to a movement of the joints in the prosthetic device.

        
%
% Introduce the new possible approach (task-space synergies) and why it could be useful: human UL trajectory planning in task-space, able-bodied like motor behaviour.
%
Another possible synergy realisation, which is yet to be considered in prosthetic interfaces, are task-space synergies \cite{Zeestraten2017}. In the upper-limb prosthetic case, these relate the motion of the joints in the residual limb to a motion of the hand. These could have an advantage over joint-space synergies in terms of the resultant upper-limb motor behaviour, as it is theorised that upper-limb motion planning is done in task-space \cite{Uno1989, Wolpert1995, Flash2013, Kistemaker2014}. From a robotics perspective, a task-space synergy can be generated using the manipulator's Jacobian \cite{Murray1994}. Assuming that knowledge of the initial conditions and the desired end-effector (hand) motion is available, then it is possible to find a relationship between the angular velocities of all the joints in the arm. However, in the prosthetic case, knowing the desired hand motion before execution of the task is a challenge as this is only known to the human. While there are multiple approaches that attempt to solve this problem through additional information sources, this remains a challenge from a practical perspective. Regardless of the method used for the realisation of the synergistic prosthetic interface, their effects on motor behaviour are not widely understood due to the limited number of studies in the field to date.

%
% Limitations of studies to date: lack of analysis of motor bevhaiour (movement patterns).
%
Studies of synergistic prosthetic devices thus far have largely focused on evaluating performance of the task \cite{Kaliki2013, Blana2016, Alshammary2016}, with a few also evaluating their effects on the quantity of compensation motion \cite{Alshammary2018, Merad2016a, Merad2018}. Significant drive behind the study of synergies in transhumeral prostheses is based on the idea that these allow for natural able-bodied motion. Quality of motion and movement patterns are significant factors in assessing upper limb motor function and behaviour, and are typically used to evaluate recovery in rehabilitation environments \cite{Balasubramanian2012b, Balasubramanian2012, DeLosReyes-Guzman2014}. However, some measures of quality of motion have only been considered as metrics for evaluating the effectiveness of a synergistic prosthetic elbow in \cite{Legrand2018}. Assessing the effects of synergistic prosthetic interfaces on motor behaviour, both in terms of quality of motion and movement patterns, is important in order to establish how these compare to able-bodied motion and whether they are effective at restoring natural motion.

%
% Contributions of this paper
%
This paper presents a set of metrics to evaluate task performance, quality of motion, and motor behaviour in the context of synergistic prostheses. These metrics are then used in a study of quality of motion and movement patterns on able-bodied subjects using a virtual prosthetic elbow with different prosthetic interfaces (traditional and synergistic) in a Virtual Reality Environment. The objective of the study is to determine how synergistic prosthetic interfaces, both in joint-space and task-space, perform in comparison to traditional prosthetic interfaces in terms of their capability to restore able-bodied motor behaviour. Lastly, given that task-space synergies are yet to be considered for transhumeral prosthetic applications, a novel method to realise these synergies in the context of the application is presented.


%
% Organisation
%
The paper is organised as follows. First, the proposed method to realise task-space kinematic synergies in trashumeral prostheses is presented. This method is based on traditional robotics methodologies. Then the metrics proposed for evaluating motor behaviour and performance in a prosthetic setting are presented; followed by the experimental methodology used to study the effects of synergistic prosthetic interfaces on motor behaviour. Lastly, results of the study are presented and discussed, which show that synergistic interfaces achieve closer to able-bodied-like motor behaviour in prosthesis users than the traditional surface electromyography based interface.

%
% Notation
%
The following notation is used throughout the paper. The set of real numbers is denoted as $\Real$, the set of positive real numbers is denoted as $\RealPos$. The left hand superscript $\frameOfRef{R}\xv$ is used to indicate the frame of reference $\{R\}$ of the vector $\xv$. The right hand superscript $x^{i}$ is used to indicate the iteration domain, such that $x^{i}$ indicates the $i$th iteration of $x$. $\| \cdot \|_2$ represents the Euclidean norm. $\rv\times\pv$ represents the cross product between vectors $\rv$ and $\pv$.
%$\mu_t(\cdot)$ represents the mean over the time domain while $\mu_i(\cdot)$ represents the mean over the task iteration domain.

==> old/1_intro_vTS.tex <==
%
% Introduction
%
\section{Introduction}
%
%

\textbf{Introduce the challenge of performing ADLs with current prostheses.}

%
% What is the main challenge that we are studying in this paper?
% Coordinated motion is required for ADLs.
% This is not possible with current prostheses.
%
Coordinated motion of the joints in the upper limb is required for most Activities of Daily Living (ADLs). Carrying out these ADLs using current upper-limb prosthesis is a challenge as these devices are only capable of sequential Degree of Freedom (DOF) motion \cite{Fougner2012}, i.e. one joint at a time. This is largely due to the limitations of the human-prosthetic interfaces (referred to as HPIs henceforth) available \cite{Biddiss2007}.


\textbf{Introduce synergies in prosthetics and advantages.}

%
% What is a possible solution for this challenge in the literature?
% A novel kinematic synergy based HPI allows for coordinated motion.
%
In the context of upper-limb prostheses, novel experimental HPIs, such as kinematic synergies and pattern recognition based interfaces \cite{Alshammary2018,Ortiz-Catalan2014}, have permitted the coordinated motion of the DOFs in a prosthesis with those of the residual limb. Synergistic HPIs in upper-limb prostheses explicitly enable the coordinated human-prosthetic arm motion required by ADLs; where motion-based synergistic interfaces determine the motion of the prosthetic device as a function of the motion the residual limb \cite{Akhtar2017}. This allows the complex coordinated motion that is otherwise not possible with traditional surface electromyography (sEMG) based interfaces.
%
% Describe the current method used to realise synergies in transhumeral prosthetics: joint-space synergies
The typical realisation of synergies in prosthetic interfaces are joint-space synergies \cite{Akhtar2017, Kaliki2013, Blana2016, Legrand2018, Alshammary2018, Garcia-Rosas2019}, where the motion of the joints in the residual limb are related to a movement of the joints in the prosthetic device.

\textbf{Review of joint-space synergies to highlight challenges with current methods.}

%
% What are the limitations of this solution?
% Synergies are individual and task/path dependent.
%
Joint-space synergies, however, also have their limitations. Most of the current methods to generate the synergies require full arm motion data, typically gathered from able-bodied subjects \cite{Khalil2013, Legrand2018}; thus introducing its own set of challenges \cite{Merad2018}. Moreover, joint-space synergies have been observed to be dependent to human motor behaviour and preference, and the task \cite{Garcia-Rosas2018EMBC, Merad2018, Gottlieb1997}. These dependencies have also been shown to occur on able-bodied individuals \cite{Bockemuhl2010}. While a method to address the dependency on human motor behaviour was presented in \cite{Garcia-Rosas2019}, the dependency on the task remains a challenge. For instance, joint-space synergy-based HPIs have only been considered for pre-defined starting positions with the ability to reach multiple targets \cite{Legrand2018, Akhtar2017, Blana2016}; however, it was observed that the generated synergies depend on the pre-defined starting position. Yet, reaching motion is constituted of arbitrary start and end positions, making it particularly challenging.


\textbf{Review of EMG + Synergy with autonomous switching:}

An attempt to address the challenge of reaching from-and-to arbitrary positions with a synergistic prosthetic elbow was presented in \cite{Alshammary2018}. There a joint-space shoulder-elbow synergy was combined with sEMG to control a virtual prosthetic elbow and hand, where sEMG allowed the user to adjust the elbow extension when the synergy was not sufficiently accurate for the task. The study, however, also included a motion-based switching mechanism between the elbow joint and the prosthetic hand. As such, while the results showed that with the method proposed therein the time required to perform the task was significantly reduced and there was significant change in compensation motion, it was not possible to discern whether the task time difference was due to the synergy component or the automated elbow-hand switching mechanism.


\textbf{Introduce the task-space synergy concept:}

Another possible synergy realisation, which is yet to be considered in prosthetic interfaces, are task-space synergies \cite{Zeestraten2017}. In the upper-limb prosthetic case, these explicitly relate the motion of the joints in the residual limb to a motion of the hand. These could have an advantage over joint-space synergies in terms of the resultant upper-limb motor behaviour, as it is theorised that upper-limb motion planning is done in task-space \cite{Uno1989, Wolpert1995, Flash2013, Kistemaker2014}. Moreover, as reaching tasks can be normalised such that the hand path is invariant of the start and end positions \cite{Yang2002}, it may be possible to generalise the synergy. Using traditional robotics tools, a task-space synergy can be generated using the manipulator's Jacobian \cite{Murray1994}. Assuming that knowledge of the initial conditions and the desired end-effector (hand) motion is available, then it is possible to find a relationship between the angular velocities of all the joints in the arm. However, in the prosthetic case, knowing the desired hand motion before execution of the task is a challenge as this is only known to the human. While there are multiple approaches that attempt to solve this problem through additional information sources, this remains a challenge from a practical perspective.

\textbf{In this paper...:}

This paper presents a realisation of a task-space synergy for upper-limb HPIs in the context of elbow prostheses and forward reaching motion. The proposed method takes a practical application perspective to address the changellenge of arbitrary point-to-point reaching motion by constraining and normalising the desired hand motion, and leveraging the voluntary information that can obtained from a prosthesis user in order to achieve arbitrary point-to-point forward hand motion. The proposed method is then compared in a virtual reality environment against able-bodied motion, traditional sEMG, and joint-space synergies under the same controlled conditions.

%
% Organisation
%
The paper is organised as follows. First, the proposed method to realise task-space kinematic synergies in trashumeral prostheses is presented. This method is based on traditional robotics methodologies. Then the metrics used for evaluating human-prosthesis motor behaviour and performance are presented; followed by the experimental methodology used to study the resultant motor behaviour and task performance. Lastly, results of the study are presented and discussed, which show that both task-space and joint-space synergistic interfaces achieve closer to able-bodied-like motor behaviour and task performance in prosthesis users than the traditional surface electromyography based interface.

%
% Notation
%
The following notation is used throughout the paper. The set of real numbers is denoted as $\Real$, the set of positive real numbers is denoted as $\RealPos$. The left hand superscript $\frameOfRef{R}\xv$ is used to indicate the frame of reference $\{R\}$ of the vector $\xv$. The right hand superscript $x^{i}$ is used to indicate the iteration domain, such that $x^{i}$ indicates the $i$th iteration of $x$. $\| \cdot \|_2$ represents the Euclidean norm. $\rv\times\pv$ represents the cross product between vectors $\rv$ and $\pv$.

==> old/2_formulation.tex <==
%
% Problem formulation
%
\section{Task-space Synergy Problem formulation}
%
% Formulate in problem in terms of the kinematic analysis
%
The objective of a task-space kinematic synergy in the context of upper-limb prosthetics is to find the motion of the prosthesis given the motion of the residual limb and the desired hand motion, which is given by the task.
Consider the traditional problem of determining a robot's end effector motion from the motion of its joints \cite{Murray1994} applied to the human-prosthesis arm. Assuming that knowledge of the initial conditions and the desired hand motion ($\vv$), then it is possible to find a relationship between the angular velocities of the residual limb joints and the prosthesis joints, $\qvd_s$ (shoulder) and $\qvd_e$ (elbow) respectively.
From the kinematic information of the arm, the following relationship between hand path velocity and joint angular position and velocities is known
\begin{equation}
    \vv = \Jacob(\qv_s,\qv_e)\begin{bmatrix} \qvd_s & \qvd_e \end{bmatrix}^T,
\end{equation}
where $\vv\in\Real^3$ is the hand velocity in task-space. $\qv_s$ and $\qvd_s$ represent residual limb joint angular displacement and velocity respectively, for the transhumeral amputation case $\qv_s\in\Real^3$ and $\qvd_s\in\Real^3$. $\qv_e$ and $\qvd_e$ represent prosthesis joint angular displacement and velocity respectively. $\mcl{J}(\qv_s,\qv_e)$ is the arm Jacobian. For the elbow prosthesis case $\qv_s\in\Real$ and $\qvd_s\in\Real$.

However, in the prosthetic case, knowing the desired hand motion ($\vv$) before execution of the task is a challenge as this is only known to the human. While there are multiple approaches that attempt to solve this problem through additional information sources, such as with Brain-Machine Interfaces \cite{Randazzo2015}, it is possible to constrain the task instead.

Here, the task constraint was chosen by taking inspiration from the synergistic motion analysis literature. The following contributions were found to be most relevant to the problem considered. Reaching motion can be normalised such that the hand path is invariant of the start and end positions \cite{Yang2002}. Forward reaching motion has been found to be most significantly related to the synergy between shoulder and elbow flexion/extension \cite{Bockemuhl2010}.

Given that a shoulder-elbow synergy is being considered, and the most significant synergistic relationship between these two appears during forward reaching motion, the task can be constrained to a forward reaching motion. Then it is possible to define a normalised forward reaching path to be used on any arbitrary point-to-point direction. Such that the user only needs to determine the direction of motion immediately prior to the reaching motion. While this restricts the admissible path to a subset of the full range of able-bodied arm motion, it is important to highlight the existence of the trade-off between practical functionality and generality of the approach.

Figure \ref{fig:reaching} presents an example of a target reaching task. By first re-positioning the hand to be aligned with the target on a forward reaching path (Figure \ref{fig:reaching1}), then the synergy can coordinate the motion of prosthetic elbow with that of the residual limb in order to to move the hand linearly towards the target, as if sliding on the path. This is represented in Figure \ref{fig:reaching2}, where the vector from the shoulder joint to the hand ($\rv_{SH}$) defines the direction of the forward reaching motion. Figure \ref{fig:reaching3} presents the proposed simplified geometry, along with frames of reference, to be used to define the desired hand path. The methodology followed to achieve the desired hand motion through a task-space kinematic synergy is presented next.

\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching1.png}
    \caption{Target reaching example. The green dotted line shows the shortest path to target. The orange dotted line the forward straight reaching path. The reference frame represented by the subscript $r$ has its origin at the shoulder with the $x$-axis pointing forward.}
    \label{fig:reaching1}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching2.png}
    \caption{Simplified geometry for a reaching task by re-positioning the hand. The hand slides across the forward reaching path. The $x_s$-$z_s$ plane is parallel to the ground.}
    \label{fig:reaching2}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching3.png}
    \caption{Definition of the direction of motion ($\{D\}$) and hand ($\{H\}$) frames that determine the forward reaching motion. The direction frame is defined by the triangle created by the shoulder (S), elbow (E), and hand (H) joints and it has its origin at the shoulder joint.}
    \label{fig:reaching3}
\end{subfigure}
\caption{Formulation of the forward reaching task and reference motion for the task-space synergy.}
\label{fig:reaching}
\end{figure*}

==> old/3_synergy.tex <==
%
% Task-space kinematic synergy
%
\section{A Task-space Kinematic Synergy}
The objective of a task-space kinematic synergy, in the context of reaching tasks in upper-limb prosthetics, is to determine the motion of the prosthesis given the motion of the residual limb and the desired hand path. However, knowing the exact desired hand path before execution of the task is a challenge as information on the desired target is only known to the prosthesis user. Another possibility is to constrain the operation of the synergy to specific reaching movements, sub-tasks, which can be initiated by the user. 

The case of a point-to-point forward reaching sub-task, and its task-space synergy, using a transhumeral prostheses is presented herein. The following contributions were found to be most relevant to the problem under consideration. Forward reaching motion can be normalised such that the hand path is invariant of the start and end positions \cite{Yang2002}. Forward reaching motion has been found to be most significantly related to the synergy between shoulder and elbow flexion/extension \cite{Bockemuhl2010}.

Based on \cite{Yang2002}, it is possible to define a normalised forward reaching path to be used on any arbitrary point-to-point direction, such that the user only needs to determine the direction of motion immediately prior to the reaching motion. While this restricts the admissible path to a subset of the full range of able-bodied arm motion, it is important to highlight the existence of the trade-off between practical functionality and generality of the approach. Based on \cite{Bockemuhl2010}, a shoulder-elbow flexion synergy is sufficient to achieve a forward reaching movement, where the other degrees of freedom in the arm determine which is the forward direction of the reaching movement.

\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching1.png}
    \caption{Target reaching example. The green dotted line shows the shortest path to target. The orange dotted line the forward straight reaching path. The reference frame represented by the subscript $r$ has its origin at the shoulder with the $x$-axis pointing forward.}
    \label{fig:reaching1}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching2.png}
    \caption{Simplified geometry for a reaching task by re-positioning the hand. The hand slides across the forward reaching path. The $x_r$-$z_r$ plane is parallel to the ground.}
    \label{fig:reaching2}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching3.png}
    \caption{Definition of the direction of motion ($\{D\}$) and hand ($\{H\}$) frames that determine the forward reaching motion. The direction frame is defined by the triangle created by the shoulder (S), elbow (E), and hand (H) joints and it has its origin at the shoulder joint.}
    \label{fig:reaching3}
\end{subfigure}
\caption{Formulation of the forward reaching task and reference motion for the task-space synergy.}
\label{fig:reaching}
\end{figure*}

Figure \ref{fig:reaching} presents an example of a target reaching task. By first re-positioning the hand to be aligned with the target on a forward reaching path (Figure \ref{fig:reaching1}), then the synergy can coordinate the motion of prosthetic elbow with that of the residual limb to move the hand linearly towards the target, as if sliding on the path. This is represented in Figure \ref{fig:reaching2}, where the vector from the shoulder joint to the hand ($\rv_{SH}$) defines the direction of the forward reaching motion. Figure \ref{fig:reaching3} presents the proposed simplified geometry, along with frames of reference, to be used to define the desired hand path.

The methodology followed to achieve the desired hand motion through a task-space kinematic synergy is presented next. Let $\vv\in\Real^3$ be the hand velocity in task-space. $\qv_s$ and $\qvd_s$ are the residual limb joint angular displacement and velocity respectively, for the transhumeral amputation case $\qv_s\in\Real^3$ and $\qvd_s\in\Real^3$. $\qv_e$ and $\qvd_e$ represent prosthesis joint angular displacement and velocity respectively, for the elbow prosthesis case $\qv_e\in\Real$ and $\qvd_e\in\Real$. $\mcl{J}(\qv_s,\qv_e)$ is the human-prosthetic arm Jacobian.

First, the user pre-positions the hand on the direction of motion path while the prosthesis is disabled, and then enables (or calibrates) the task-space synergy. The enabling can be done through additional interface modalities, such as sEMG, where the user can voluntarily manipulate the signal. Then, in order to obtain the synergy between the shoulder (residual limb) and the hand motion (prosthesis) for a given start position the following steps are taken:
\renewcommand{\labelenumi}{\Alph{enumi}.}
\begin{enumerate}
    \item Determine the forward reaching task direction of motion reference frame (frame $\{D\}$).
    \item Determine the frame transformation ($\transform{D}{R}R$) in order to express shoulder and elbow joint angular displacement with reference to frame $\{D\}$.
    \item Determine the arm Jacobian and the hand motion constraint on $^{D}\dot{x}_h$.
    \item Solve for $\qvd_e$ as a function of $\qv_s$, $\qv_e$, and $\qvd_s$ to determine the elbow motion reference that satisfies the desired task-space synergy.
\end{enumerate}

\begin{remark}
It is important to note that while the motion coupling is between the residual limb and the hand, the prosthesis is actuated by the elbow. Thus it is necessary to solve for the elbow motion that will satisfy the desired hand motion. This is done through the arm Jacobian.
\end{remark}

The following assumptions are used:
\begin{assumption}
    The angular position and velocities of the residual limb are measurable. 
\end{assumption}
\begin{remark}
    Intertial Measurement Unit (IMU)-based measurements of residual limb motion have been demonstrated for synergistic elbow prostheses in \cite{Alshammary2018, Merad2016a}.
\end{remark}
\begin{assumption}
    The joint-to-joint distances of the human-prosthesis arm are known.
\end{assumption}
\begin{remark}
    Joint-to-joint distances of the arm are required to determine the arm Jacobian. Moreover, knowledge of the dimensions of the the user's residual limb and prosthesis, along with measurements of joint position, allow the computation of the hand pose ($\pv$) using forward kinematics.
\end{remark}
The steps of the proposed method to determine the task-space synergy are detailed next. A video explanation can be found in \textbf{ADD EXPLANATION VIDEO}.
%
% D frame
%
\subsection{Direction of Motion Reference Frame} 
The direction of motion reference frame determines the direction of the forward reaching task as exemplified in Figure \ref{fig:reaching2}. Let a reference frame (frame $\{R\}$) be located at the center of the shoulder joint with the $x$-axis pointing forward and the $y$-axis upwards w.r.t. the upper body. Let the origin of the direction of motion frame (frame \{D\}) be located at the center of the shoulder joint. The direction of motion frame w.r.t. the reference frame is defined as follows:
    \begin{itemize}
        \item $x_d$-axis: The unit vector given in the direction from the shoulder joint center to the initial hand position $\frameOfRef{R}\pv$.
        \begin{equation}
            \frameOfRef{R}\xv_d = \frac{\frameOfRef{R}\pv}{\|\frameOfRef{R}\pv\|_2}
        \end{equation}
        \item $z_d$-axis: The unit vector perpendicular to the plane given by the S-E-H triangle, in the direction of $z_r$. This can be defined by
        \begin{equation}
            \frameOfRef{R}\zv_d =  \frac{ \frameOfRef{R}\rv_{RE} \times \frameOfRef{R}\xv_d }{\|\frameOfRef{R}\rv_{RE} \times \frameOfRef{R}\xv_d\|_2}
        \end{equation}
        where $\frameOfRef{R}\rv_{RE}$ is the vector from the shoulder to the elbow joint.
        \item $y_d$-axis: Follows the right hand rule.
    \end{itemize}
With this the direction of motion reference frame $\{D\}$ is defined and motion of the arm and hand can be expressed with it as reference. This concludes step A. 

%
% Frame transformation
%
\subsection{Frame Transformation} 
Assuming that measured data is obtained in frame $\{R\}$ then it is necessary to transform these angles to the task frame $\{D\}$. This assumption arises from the common use of relative measurements from two IMUs to produce residual limb pose measurements \cite{Alshammary2018, Merad2016a}. This transformation can be performed through the Euler angles ($\alpha$, $\beta$, $\gamma$) in a Y-X-Z sequence. The transformation angles can be obtained as follows:
\begin{itemize}
    \item $\alpha$: The first rotation is along the $y_r$-axis. $\alpha$ can be obtained from $\frameOfRef{R}\xv_d$, as given by:
    \begin{equation}
        \alpha = \tan^{-1}{\left ( \frac{\frameOfRef{R}\xv_{d,x}}{\frameOfRef{R}\xv_{d,z}} \right )},
    \end{equation}
    where $\frameOfRef{R}\xv_{d,x}$ and $\frameOfRef{R}\xv_{d,z}$ are the $x$ and $z$ components of $\frameOfRef{R}\xv_{d}$.
    \item $\beta$: The second rotation is along the $x_r$-axis. $\beta$ can be obtained from $\frameOfRef{R}\zv_d$, as given by:
    \begin{equation}
        \beta = \tan^{-1}{\left ( \frac{\frameOfRef{R}\zv_{d,y}}{\frameOfRef{R}\zv_{d,z}} \right )}.
    \end{equation}
    \item $\gamma$: The last rotation is along the $z_r$-axis. $\gamma$ can be obtained from $\frameOfRef{R}\xv_d$, as given by:
    \begin{equation}
        \gamma = \tan^{-1}{\left ( \frac{\frameOfRef{R}\xv_{d,y}}{\frameOfRef{R}\xv_{d,x}} \right )}.
    \end{equation}
\end{itemize}

Then the frame transformation is given by
\begin{equation}
    \transform{D}{R}R = R_{y}(\alpha)R_{x}(\beta)R_{z}(\gamma),
\end{equation}
where $R_{x}(\alpha)$ is an $x$-axis standard rotation of the given angle $\alpha$. Thus it is possible to transform arm motion data from the reference frame $\{R\}$ to the task frame $\{D\}$. This concludes step B.

%
% Jacobian
%
\subsection{Arm Jacobian}
By performing the adequate transformations, as previously presented, the forward reaching task can be simplified to a 2D task on the $x-y$ plane of the $D$ frame. This simplifies the kinematics required for the synergy to those of a 2-DOF planar arm. The differential kinematics of the simplified arm are well known and given by \cite{Murray1994}:
\begin{subequations}
\label{eq:simpDiffKine}
\begin{align}
    \bar{\vv} = \begin{bmatrix} ^{D}\dot{x}_h \\ ^{D}\dot{y}_h \end{bmatrix} &= \bar{\Jacob}(\bar{q}_s,\bar{q}_e)\begin{bmatrix} \dot{q}_s \\ \dot{q}_e \end{bmatrix},\\
    \bar{\Jacob}(\bar{q}_s,\bar{q}_e) &= \begin{bmatrix}
    -\ell_{u} S_s - \ell_{l} S_{se} & -\ell_{l} S_{se}\\
    \ell_{u} C_s + \ell_{l} C_{se} & \ell_{l} C_{se}
    \end{bmatrix}.
\end{align}
\end{subequations}
where $C_s = \cos{(\bar{q}_{s})}$, $S_s = \sin{(\bar{q}_{s})}$, $C_{se} = \cos{(\bar{q}_{s} + \bar{q}_{e})}$, $S_{se} = \sin{(\bar{q}_{s} + \bar{q}_{e})}$, $\bar{q}_{s} = \frameOfRef{D}q_{s}$, and $\bar{q}_{e} = \frameOfRef{D}q_{e}$. $\ell_{u}$and $\ell_{l}$ are the lengths of the upper and lower arm respectively. This concludes step C.

%
% Synergy
%
\subsection{Elbow Motion Reference}
As previously discussed, through the simplification of the task only forward reaching motion is required along the direction of motion plane, i.e. only motion along the $x_d$-axis. This means that it is desired to satisfy the constraint $^{D}\dot{y}_h = 0$. With this constraint in consideration, it is possible to solve for the desired elbow velocity $\dot{q}_e$ from Equation (\ref{eq:simpDiffKine}), such that
\begin{equation}
\label{eq:taskSpaceSynergy}
    \dot{q}_e = -\ell_{l} C^{-1}_{se}(\ell_{u} C_s + \ell_{l} C_{se})\dot{q}_s.
\end{equation}
It is important to note that a singularity exists when $\bar{q}_{s} + \bar{q}_{e} = n\pi/2$, $n = 1, 3, \cdots$.  These singularities occur This can be avoided by limiting the range of motion of the elbow. This concludes step D, and the Task-space Synergy method.


==> old/4_metrics.tex <==
%
% Metrics for evaluating motor behaviour and performance
%
\section{Metrics for Evaluating Motor Behaviour and Performance}
Three categories of metrics are used in this paper to evaluate the subject's performance of the task and the effects of prosthetic interfaces on the following aspects of reaching motion: task performance, quality of motion, and motor behaviour.
%
% Task
%
\subsection{Task Performance Metrics}
\subsubsection{Task completion time ($t_f^{\mu}$)}
This metric determines the effects of prosthetic interfaces on the time required to complete the task. As this metric is commonly used in the literature, it is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature. The mean task time ($t_f^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:taskTime}
    t_f^{\mu} = \sum_{i=1}^{I}\frac{t_f^i}{I},
\end{equation}
where $t_f^i$ is the task end time for a given iteration $i>0$ and $I\in\RealPos$ is the total number of iterations.
\subsubsection{Accuracy ($\delta^{\mu}$)}
This metric is used to verify that the task is being performed adequately. Let the desired hand target position be given by $\bar{\pv}_f$. Then the mean accuracy ($\delta^{\mu}$) over iterations of the task is given by:
\begin{equation}
\label{eq:accuracy}
    \delta^{\mu} = \sum_{i=1}^{I}\frac{\|\bar{\pv}_f - \pv_f^i\|_2}{I},
\end{equation}
where $\pv_f^i$ is the hand final position for a given iteration $i$.

%
% Quality of motion
%
\subsection{Quality of Motion Metrics}
Two metrics for quality of motion are considered in this paper: path smoothness and variability.

\subsubsection{Path smoothness ($\eta$)}
Continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL) is used as the metric for smoothness \cite{Balasubramanian2012a} due to its characteristics which include sensitivity to changes in motor characteristics, robustness to measurement noise, provides a monotonic response (increase in movement complexity, increase in SAL), and is dimensionless.

Let $\xvd(t)$ be the hand ($\pvd(t)$) or joints ($\qvd(t)$) speed vector, such that the speed profile of the hand or joints is given by $v(t) = \| \xvd(t) \|_2$. $V(\omega)$ is the Fourier magnitude spectrum of $v(t)$, where $\omega\in \begin{bmatrix} 0,\omega_c \end{bmatrix}$ and $\omega_c = 40 rad/s$ which corresponds to the frequency range of motion of the human arm. Then, the spectral arc length of the path $(\eta)$ is given by \cite{Balasubramanian2012a}:
\begin{subequations}
\label{eq:smoothness}
\begin{align}
    \hat{V}(\omega) &= \frac{V(\omega)}{V(0)}, \\
    \eta &= -\int_{0}^{\omega_c} \sqrt{ \begin{pmatrix}
    \frac{1}{\omega_c}
    \end{pmatrix}^2 + \begin{pmatrix}
    \frac{ \partial\hat{V}(\omega) }{ \partial\omega }
    \end{pmatrix}^2} d\omega.
\end{align}
\end{subequations}
    
\subsubsection{Path variability ($\sigma_{\mu}$)}
Low path variability, both of the hand and joints, is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint) is used as the metric for path variability.

The hand/joint path variability metric ($\sigma_{\mu}$) is defined herein by the mean standard deviation of the hand/joint path across the time domain as follows. Let the hand or joint path vector for a given iteration $i$ be $\xv^i(t_s n)$ and the mean path vector over the $I$ number of iterations be $\xv^{\mu}(t_s n)$. $t_s > 0$ is the path sampling time, $n>0$ the sample number, and $N\in\RealPos$ is the total number of samples.
\begin{subequations}
\label{eq:handSTD}
\begin{align}
    \sigmav(t_s n) &= \sqrt{ \frac{\sum_{i=1}^{I}(\xv^i(t_s n)   - \xv^{\mu}(t_s n) )^2 }{I} }, \\
    \sigma_{\mu} &= \sum_{n=0}^{N}\frac{\sigmav(t_s n)}{N}.
\end{align}
\end{subequations}

%
% Motor behaviour
%
\subsection{Motor Behaviour Metrics}
Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion. The metrics used in this paper use individual able-bodied motion as the point of reference for each subject. To provide a deeper analysis of motor behaviour, particularly with respect to movement patterns, individual behaviour will also be analysed in the results section in addition to the metrics presented next.

\subsubsection{Path difference ($\Delta_{\mu}$)}
This metric evaluates the difference between the mean able-bodied hand/joint path and the mean prosthetic hand/joint path. This is used to determine the closeness of the resultant prosthetic motor behaviour to the individual's natural able-bodied motor behaviour. Let the mean hand/joint path for the able-bodied case ($AB$) be given by $\xv_{AB}^{\mu}(t_s n)$ and the mean path for the prosthetic case ($PC$) given by $\xv_{PC}^{\mu}(t_s n)$. The path difference ($\Delta_{\mu}$) is defined as the mean absolute difference between the mean paths across the time domain as follows.

\begin{subequations}
\label{eq:handDiff}
\begin{align}
    \Deltav(t_s n) &=  \left | \xv_{AB}^{\mu}(t_s n)- \xv_{PC}^{\mu}(t_s n) \right |, \\
    \Delta_{\mu} &=  \sum_{n=0}^{N}\frac{\| \Deltav_p(t_s n) \|_2}{N}.
\end{align}
\end{subequations}

\subsubsection{Upper-body displacement ($\phi^{\mu}$)}
This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Some level of upper-body motion is also part of natural able-bodied motion during reaching tasks. Let the position of the part of the upper-body to be analysed be given by $\pv_{UB}(t)\in\Real^3$. The metric is defined as follows:
\begin{subequations}
\label{eq:motionMagnitude}
\begin{align}
    \phiv^i &=  \| \pv_{UB}^i(t_f) - \pv_{UB}^i(0)\|_2, \\
    \phi^{\mu} &=  \sum_{i=1}^{I}\frac{\phiv^i }{I}.
\end{align}
\end{subequations}


==> old/4_metrics_vShort.tex <==
%
% Metrics for evaluating motor behaviour and performance
%
\section{Metrics for Evaluating Motor Behaviour and Performance}
Three categories of metrics are used in this paper to evaluate the subject's performance of the task and the effects of prosthetic interfaces on the following aspects of reaching motion: task performance, quality of motion, and motor behaviour.
%
% Task
%
\subsection{Task Performance Metrics}
\subsubsection{Task completion time ($t_f^{\mu}$)}
The mean task time over iterations of the task is used to determine the effects of prosthetic interfaces on the time required to complete the task. As this metric is commonly used in the literature, it is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature.
\subsubsection{Accuracy ($\delta^{\mu}$)}
The mean reach accuracy over iterations of the task is used to verify that the task is being performed adequately.

%
% Quality of motion
%
\subsection{Quality of Motion Metrics}
Two metrics for quality of motion are considered in this paper: path smoothness and variability.

\subsubsection{Path smoothness ($\eta$)}
Continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL) is used as the metric for smoothness \cite{Balasubramanian2012a} due to its characteristics which include sensitivity to changes in motor characteristics, robustness to measurement noise, provides a monotonic response (increase in movement complexity, increase in SAL), and is dimensionless.
    
\subsubsection{Path variability ($\sigma_{\mu}$)}
Low path variability, both of the hand and joints, is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint) is used as the metric for path variability.

%
% Motor behaviour
%
\subsection{Motor Behaviour Metrics}
Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion. The metrics used in this paper use individual able-bodied motion as the point of reference for each subject. To provide a deeper analysis of motor behaviour, particularly with respect to movement patterns, individual behaviour will also be analysed in the results section in addition to the metrics presented next.

\subsubsection{Path difference ($\Delta_{\mu}$)}
This metric evaluates the difference between the mean able-bodied hand/joint path and the mean prosthetic hand/joint path. This is used to determine the closeness of the resultant prosthetic motor behaviour to the individual's natural able-bodied motor behaviour. Let the mean hand/joint path for the able-bodied case ($AB$) be given by $\xv_{AB}^{\mu}(t_s n)$ and the mean path for the prosthetic case ($PC$) given by $\xv_{PC}^{\mu}(t_s n)$. The path difference ($\Delta_{\mu}$) is defined as the mean absolute difference between the mean paths across the time domain as follows.

\begin{subequations}
\label{eq:handDiff}
\begin{align}
    \Deltav(t_s n) &=  \left | \xv_{AB}^{\mu}(t_s n)- \xv_{PC}^{\mu}(t_s n) \right |, \\
    \Delta_{\mu} &=  \sum_{n=0}^{N}\frac{\| \Deltav_p(t_s n) \|_2}{N}.
\end{align}
\end{subequations}

\subsubsection{Upper-body displacement ($\phi^{\mu}$)}
This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Some level of upper-body motion is also part of natural able-bodied motion during reaching tasks.


==> old/5_methodology.tex <==
%
% Experimental methodology
%
\section{Experimental Methodology}
%
% Experiment objective
%
The objective of the experiment is to understand the effects of synergistic prosthetic interfaces on upper-limb motor behaviour, in terms of quality of motion and movement patterns, and to determine the closeness of the resultant human-prosthetsis motor behaviour with respect to natural able-bodied behaviour. The experiment was performed on able-bodied subjects in a Virtual Reality Environment (VRE) which was presented to the subjects with an HTC Vive Pro Head Mounted Display (HMD). This allowed to gather able-bodied motor behaviour data from subjects, and the virtually amputate and fit them with a virtual prosthetic device in order to analyse motor behaviour while using a prosthetic device. The focus of the experiment was on the use of the prosthetic device and how this use affects upper body and arm motion. Therefore, the prosthetic interface was simplified to reduce the cognitive burden of prosthesis use on subjects with no previous experience with such devices.


%
% Describe the experiment
%
\subsection{Experiment Description}
%
% Present the task
%
The task required subjects to pick and place an object in 3D space in the forward direction from a standing position in a VRE. Subjects were not allowed to step to perform the task. An iteration of the task was considered from when the object was grasped until the object was placed. One object start position and 4 target positions were used.

%
% Present detail on the target locations.
%
Consider the following reference frames:
\begin{enumerate}
    \item Virtual world frame of reference. This frame of reference was chosen such that for the task the x-axis represents the forward direction, the y-axis the upwards direction, and the z-axis the lateral direction. The origin was placed on the floor under the position where the subjects were standing to perform the task.
    \item Sensor frame of reference. This frame of reference is determined by the motion sensor's yaw, pitch, and roll.
\end{enumerate}
Start and target positions were normalised to each subject's height and arm length. Let a subject's arm length be represented by $\ell$ and height by $h$. The target locations, in the virtual world frame of reference, are presented in Table \ref{ta:targets}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Object start and target positions.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Target & $x (m)$ & $y (m)$ & $z (m)$  \\
        \hline
        \hline
        Start (ST)   &     $0.5\ell$     &     $0.5h$   &  0 \\
        \hline
        Close (CT)   &     $0.75\ell$    &     $0.65h$   &  0.12   \\
        \hline
        Mid (MT)   &     $1.0\ell$      &     $0.65h$   &  -0.12 \\
        \hline
        Far (FT)   &     $1.5\ell$      &     $0.65h$   &  0   \\
        \hline
        High (HT)   &     $1.0\ell$      &     $0.9h$   &  0   \\
        \hline
    \end{tabular}
    \label{ta:targets}
    %\vspace{-5mm}
\end{table}

The reasons for the choice of target locations were the following:
\begin{itemize}
    \item Start (ST): Reachable from a neutral, relaxed position with the upper-arm down and elbow bent $90\deg$.
    \item Close (CT): A target that did not require the subject to use the prosthesis to perform the task.
    \item Mid (MT): A target that could be reached through either only using arm extension or compensation motion.
    \item Far (FT): A target that required both arm extension and upper-body lean to be reached.
    \item High (HT): A target that required both arm extension and shoulder motion to be reached.
\end{itemize}
These targets allow to study different movement patterns that occur on day-to-day reaching tasks in unstructured environments. An example for start and target positions for a subject in the VRE are presented in Figure \ref{fig:sideView} and \ref{fig:subjectView}.

%
% Present detail on the modalities tested.
%
Four different modalities were considered for the experiment, 1 able-bodied and 3 transhumeral prosthetic:
\begin{itemize}
    \item Able-bodied (AB). Used as the benchmark for individual subject performance.
    \item sEMG proportional (EP). Most widely used interface modality for active prostheses. Dual-site differential sEMG activation commands the prosthetic elbow joint speed \cite{Fougner2012}.
    \item Joint-space kinematic synergy (JS). Most basic type of synergistic interface. Shoulder-elbow flexion synergy as given by $\dot{q}_e = \theta \dot{q}_s$; where $\dot{q}_e$ is the prosthetic elbow velocity, $\dot{q}_s$ the shoulder extension velocity and $\theta = 1$ the synergy parameter.
    \item Task-space kinematic synergy (TS). The proposed task-space synergy method, where the synergy is given by (\ref{eq:taskSpaceSynergy}).
\end{itemize}

The following prosthetic interface simplifications where done in order to reduce the cognitive load on the subjects and be able to focus the experiment on the motor behaviour aspect of prosthesis use:
\begin{itemize}
    \item The functionality of the prosthetic elbow was enabled with a button press instead of relying on complex sEMG switching commands, such as co-contraction, which are common place in prosthetics and are a major issue with active prostheses to date \cite{Biddiss2007a}.
    \item Grasping and releasing of the object were done automatically when the subject stopped moving the hand and was touching the object (grasp) and within the target area (release). This avoided the need to switch between elbow and hand control.
\end{itemize}


%
% Experiment set-up Figure
%
\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/TaskPOVAnnotated.png}
    \caption{Side view of the task. The object start position and target locations were normalised to the subject's height and arm length.}
    \label{fig:sideView}
\end{subfigure}
~
\begin{subfigure}[t]{0.315\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectPOVAnnotated.png}
    \caption{Subject point of view of the task. Only one target location was presented per repetition of the task and was selected randomly. Subjects were required to place the virtual hand on the orange circle before each repetition of the task.}
    \label{fig:subjectView}
\end{subfigure}

\begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectAnnotated.png}
    \caption{Subject with motion tracking sensors, elbow brace, and VR headset. Motion trackering sensors are highlighted by the yellow circles. Motion tracking sensors were placed on: C7 vertebrae, shoulder acromion, upper arm, forearm, and hand. An elbow immobiliser was used for the virtual prosthetic cases to better emulate prosthesis use. In the EMG case, two sEMG sensors were placed on the subject's forearm.}
    \label{fig:subject}
\end{subfigure} 
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/AbleAvatarAnnotated.png}
    \caption{Able-bodied VR avatar. The forearm and hand motion trackers were used to create a forearm and hand avatar for the subject while the rest of the trackers were presented only as white markers. In the able bodied case, the elbow immobiliser was inactive to allow the subject to perform the task naturally. Grasping and dropping-off of the object were performed automatically.}
    \label{fig:ableAvatar}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/ProstheticAvatarAnnotated.png}
    \caption{Prosthetic VR avatar. The upper arm motion tracker was used to create a ``residual limb'' avatar to which the virtual prosthesis was attached while the rest of the trackers were presented only as white markers. In the prosthetic cases, the elbow immobiliser was engaged and forearm and hand tracking was disabled. Grasping and dropping-off of the object were performed automatically.}
    \label{fig:prosthesisAvatar}
\end{subfigure}
\caption{Experimental platform and task set-up. (a) presents the side view of the task while (b) the subject point of view in VR. (c) presents motion tracking sensor placement. (d) and (e) present the virtual avatars for the able-bodied and prosthetic cases.}
\label{fig:taskSetup}
\end{figure*}
%
% Figure END
%

%
% Describe the protocol
%
\subsection{Experiment Protocol}
The experiment was performed on 15 able-bodied subjects, 6 female and 9 male. The age range was $[22, 34]$ and the median age $28$ years old. The experiment was performed in 2 different sessions lasting 2 hours each. Each session was done on different days, not more than a week apart. Each session tested two different modalities. The first modality tested for all subjects was AB which was used as the benchmark for individual motor behaviour. The following modalities (prosthetic-based) were randomly selected to minimise the bias introduced by the effects of learning on the data gathered. The sessions procedure is presented in Table \ref{ta:protocol}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Experiment session protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|}
        \hline
        Step & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Introduction   &     5     &     No-VR \\
        \hline
        Sensor placement   &     15   &     No-VR    \\
        \hline
        Modality 1  &     50      &     VR  \\
        \hline
        Break   &     5      &     No-VR  \\
        \hline
        Modality 2  &     50      &     VR  \\
        \hline
    \end{tabular}
    \label{ta:protocol}
    %\vspace{-5mm}
\end{table}

Each block for Modality testing consisted of 120 iterations of the task separated in 3 sets of 40 iterations. The procedure for each modality testing is presented in Table \ref{ta:modalityProtocol}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Modality testing block protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Step & Task iterations per target & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Training   &     -    &     5    &     No-VR \\
        \hline
        Practice   &     5    &     -    &     VR    \\
        \hline
        Set 1      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 2      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 3      &     10   &     -   &     VR  \\
        \hline
    \end{tabular}
    \label{ta:modalityProtocol}
    %\vspace{-5mm}
\end{table}

Only the last set of 40 iterations for each modality was used for data analysis in order to reduce the effects of motor learning on the results. Subjects were asked to use the prosthetic device as much as possible during the trials as the objective of the experiment was to analyse motor behaviour when the prosthetic device is used. Transhumeral amputation was emulated in able-bodied subjects in the VRE by using a motion sensor on the upper arm (Figure \ref{fig:subject}) which determined the motion of the virtual residual limb. A virtual prosthetic elbow, forearm, and hand were attached to the virtual residual limb. Further details on sensor placement and data gathering are presented in Section \ref{sec:dataGathering}. Figures \ref{fig:ableAvatar} and \ref{fig:prosthesisAvatar} show the VRE avatars for the able-bodied and prosthetic cases. During the Training block of the experiment subjects were instructed outside the VRE on how to use the prosthetic interface and were allowed to familiarise themselves with it. This was done by presenting a third person view of the virtual residual limb and prosthetic device on a screen. The procedure was approved by the University of Melbourne Human Research Ethics Committee, project number 1750711.1. Informed consent was received from all subjects in the study. A video of the experimetal platform can be found in \textbf{ADD VIDEO OF EXPERIMENT}.

%
% Describe the protocol
%
\subsection{Data Gathering}
\label{sec:dataGathering}
Upper-body, arm, and hand position and orientation in 3D space was gathered using motion trackers. Muscle activation, used for the EP modality, was gathered using surface EMG electrodes. A summary of sensor type, location, and modalities where they were used are presented in Table \ref{ta:sensorInfo}. sEMG electrodes were placed on the forearm as the elbow brace interfered with the biceps/triceps eletrode placement used by transhumeral amputees. Furthermore, it was found that able-bodied subjects had a difficulty isolating biceps and triceps activation, which is required for the effective use of the EP modality. While this electrode position does not reflect the physiological placement of sEMG sensors for transhumeral prostheses, it can provide comparable functional capabilities.



%
% Sensor placement table
%
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Sensor placement and information.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Location & Sensor type & Reference frame & Modalities \\
        \hline
        \hline
        C7 Vertebra &  Motion  & Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Shoulder &  Motion  &  Virtual world (position)  &  All \\
        acromion &          & Sensor (orientation)      & \\
        \hline
        Upper-arm &  Motion &  Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Lower-arm &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Hand    &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Forearm   &  sEMG &  -  &  EP \\
                  &       &     & \\
        \hline
    \end{tabular}
    \label{ta:sensorInfo}
    %\vspace{-5mm}
\end{table}


\subsection{Hardware Set-up}
The experiment was performed on an HTC Vive Pro HMD with the application developed in Unity3D. The experimental platform runs on an Intel Core i7-8700K processor at 3.7GHz, with 32GB RAM, and an Gigabyte GeForce GTX 1080Ti video card with 11GB GDDR5. HTC Vive Trackers were used for motion tracking, except for hand motion tracking where an HTC Vive Controller was used (an analysis of the HTC Vive system tracking capabilities can be found in \cite{Niehorster2017}). The Vive Trackers were attached directly to the subject's body using medical tape. Data gathering, and VR update were performed at 90Hz. Myoware sensors were used for sEMG data gathering with Ag-AgCl electrodes. The application used for the experiment can be downloaded from \textbf{ADD GITHUB LINK}.

==> old/5_methodology_v2.tex <==
%
% Experimental methodology
%
\section{Experimental Methodology}
%
% Experiment objective
%
The objective of the experiment was to compare the performance of the prosposed task-space synergistic prosthetic interface against able-bodied, traditional and joint-space synergistic prosthetic interfaces, in terms of task performance, quality of motion, and movement patterns. The experiment was performed on able-bodied subjects in a Virtual Reality Environment (VRE) which was presented to the subjects with an Head Mounted Display (HMD). This allowed to gather able-bodied motor behaviour data from subjects, and then virtually amputate and fit them with a virtual prosthetic device in order to analyse motor behaviour while using a prosthetic device. The focus of the experiment was on the use of the prosthetic device and how this use affects upper body and arm motion. Therefore, the prosthetic interface was simplified to reduce the cognitive burden of prosthesis use on subjects with no prior experience with such devices.

%
% Describe the experiment
%
\subsection{Experiment Description}
%
% Present the task
%
The task required subjects to pick and place an object in 3D space in the forward direction from a standing position in a VRE. Subjects were not allowed to step to perform the task. An iteration of the task was considered from when the object was grasped until the object was placed. One object start position and 4 target positions were used.

%
% Present detail on the target locations.
%
Consider the following reference frames:
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item \textit{Virtual world frame of reference.} This frame of reference was chosen such that for the task the x-axis represents the forward direction, the y-axis the upwards direction, and the z-axis the lateral direction. The origin was placed on the floor under the position where the subjects were standing to perform the task.
    \item \textit{Sensor frame of reference.} This frame of reference is determined by the motion sensor's yaw, pitch, and roll.
\end{enumerate}
Start and target positions were normalised to each subject's height and arm length. Let a subject's arm length be represented by $\ell$ and height by $h$. The target locations, in the virtual world frame of reference, are presented in Table \ref{ta:targets}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Object start and target positions.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|p{3.8cm}|}
        \hline
        Target & $x (m)$ & $y (m)$ & $z (m)$ & Comment \\
        \hline
        \hline
        Start  &     $0.5\ell$     &     $0.5h$   &  0 & Reachable from a neutral, relaxed position with the upper-arm down and elbow bent $90\deg$.\\
        \hline
        Close  &     $0.75\ell$    &     $0.65h$   &  0.12 & Reachable with upper-body motion only.  \\
        \hline
        Mid  &     $1.0\ell$      &     $0.65h$   &  -0.12 & Reachable with either upper-body motion or arm extension only. \\
        \hline
        Far  &     $1.5\ell$      &     $0.65h$   &  0 & Reachable with both upper-body motion and arm extension only.  \\
        \hline
        High  &     $1.0\ell$      &     $0.9h$   &  0  & Reachable with both upper-body motion and arm extension only. \\
        \hline
    \end{tabular}
    \label{ta:targets}
    %\vspace{-5mm}
\end{table}

%The reasons for the choice of target locations were the following:
%\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
%    \item \textit{Start (ST):} Reachable from a neutral, relaxed position with the upper-arm down and elbow bent $90\deg$.
%    \item \textit{Close (CT):} A target that did not require the subject to use the prosthesis to perform the task.
%    \item \textit{Mid (MT):} A target that could be reached through either only using arm extension or compensation motion.
%    \item \textit{Far (FT):} A target that required both arm extension and upper-body lean to be reached.
%    \item \textit{High (HT):} A target that required both arm extension and shoulder motion to be reached.
%\end{enumerate}
These targets allow to study different movement patterns that occur on day-to-day reaching tasks in unstructured environments. An example for start and target positions for a subject in the VRE are presented in Figure \ref{fig:sideView} and \ref{fig:subjectView}.

%
% Present detail on the modalities tested.
%
The following experiment modalities were considered for comparison, 1 able-bodied and 3 transhumeral prosthetic:
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item \textit{Able-bodied (AB).} Used as the benchmark for individual subject performance.
    \item \textit{sEMG proportional (EP).} Standard dual-site differential sEMG commands the prosthetic elbow joint speed \cite{Fougner2012}.
    \item \textit{Task-space kinematic synergy (TS).} The proposed task-space synergy method, where the synergy is given by (\ref{eq:taskSpaceSynergy}).
    \item \textit{Joint-space kinematic synergy (JS).} Most basic type of synergistic interface. Shoulder-elbow flexion synergy as given by $\dot{q}_e = \theta \dot{q}_s$; where $\dot{q}_e$ is the prosthetic elbow velocity, $\dot{q}_s$ the shoulder extension velocity and $\theta = 1$ the synergy parameter.
\end{enumerate}

The following prosthetic interface simplifications where done in order to reduce the cognitive load on the subjects and be able to focus the experiment on the motor behaviour aspect of prosthesis use:
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item The functionality of the prosthetic elbow was enabled with a button press instead of relying on complex sEMG switching commands, such as co-contraction, which are common place in prosthetics and are a major issue with active prostheses to date \cite{Biddiss2007a}.
    \item Grasping and releasing of the object were done automatically when the subject stopped moving the hand and was touching the object (grasp) and within the target area (release). This avoided the need to switch between elbow and hand control.
\end{enumerate}


%
% Experiment set-up Figure
%
\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.29\textwidth}
    \includegraphics[width=\textwidth]{Figures/TaskPOVAnnotated.png}
    \caption{Side view of the task. The object start position and target locations were normalised to the subject's height and arm length.}
    \label{fig:sideView}
\end{subfigure}
~
\begin{subfigure}[t]{0.305\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectPOVAnnotated.png}
    \caption{Subject point of view of the task. Only one target location was presented per repetition of the task. Subjects were required to place the virtual hand on the orange circle before each repetition of the task.}
    \label{fig:subjectView}
\end{subfigure}

\begin{subfigure}[t]{0.30\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectAnnotated.png}
    \caption{Subject with motion tracking sensors, elbow brace, and VR headset. Motion tracking sensors were placed on: C7 vertebrae, shoulder acromion, upper arm, forearm, and hand. An elbow immobiliser was used for the virtual prosthetic cases. In the EMG case, two sEMG sensors were placed on the subject's forearm.}
    \label{fig:subject}
\end{subfigure} 
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/AbleAvatarAnnotated.png}
    \caption{Able-bodied VR avatar. Motion trackers determine the motion of the forearm and hand avatars and the white markers. The elbow immobiliser was inactive to allow the subject to perform the task naturally.}
    \label{fig:ableAvatar}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/ProstheticAvatarAnnotated.png}
    \caption{Prosthetic VR avatar. The upper arm motion tracker was used to create a ``residual limb'' avatar to which the virtual prosthesis was attached. The rest of the trackers were presented only as white markers. The elbow immobiliser was engaged, and forearm and hand tracking was disabled.}
    \label{fig:prosthesisAvatar}
\end{subfigure}
\caption{Experimental platform and task set-up. (a) presents the side view of the task while (b) the subject point of view in VR. (c) presents motion tracking sensor placement. (d) and (e) present the virtual avatars for the able-bodied and prosthetic cases.}
\label{fig:taskSetup}
\end{figure*}
%
% Figure END
%

%
% Describe the protocol
%
\subsection{Experiment Protocol}
The experiment was performed on 15 able-bodied subjects, 6 female and 9 male. The age range was $[22, 34]$ and the median age $28$ years old. The experiment was performed in two different sessions lasting two hours each. Each session was done on different days, not more than a week apart. Each session tested two different modalities. The first modality tested for all subjects was AB which was used as the benchmark for individual motor behaviour. The following modalities (prosthetic-based) were randomly selected to minimise the bias introduced by the effects of learning on the data gathered. The sessions' procedure is presented in Table \ref{ta:protocol}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Experiment session protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|}
        \hline
        Step & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Introduction   &     5     &     No-VR \\
        \hline
        Sensor placement   &     15   &     No-VR    \\
        \hline
        Modality 1  &     50      &     VR  \\
        \hline
        Break   &     5      &     No-VR  \\
        \hline
        Modality 2  &     50      &     VR  \\
        \hline
    \end{tabular}
    \label{ta:protocol}
    %\vspace{-5mm}
\end{table}

Each block of modality testing consisted of 120 iterations of the task separated into three sets of 40 iterations. The procedure for each modality testing is presented in Table \ref{ta:modalityProtocol}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Modality testing block protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Step & Task iterations per target & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Training   &     -    &     5    &     No-VR \\
        \hline
        Practice   &     5    &     -    &     VR    \\
        \hline
        Set 1      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 2      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 3      &     10   &     -   &     VR  \\
        \hline
    \end{tabular}
    \label{ta:modalityProtocol}
    %\vspace{-5mm}
\end{table}

Only the last set of 40 iterations for each modality was used for data analysis in order to reduce the effects of motor learning on the results. Subjects were asked to use the prosthetic device as much as possible during the trials as the objective of the experiment was to analyse motor behaviour when the prosthetic device is used. Transhumeral amputation was emulated in able-bodied subjects in the VRE by using a motion sensor on the upper arm (Figure \ref{fig:subject}) which determined the motion of the virtual residual limb. A virtual prosthetic elbow, forearm, and hand were attached to the virtual residual limb. Further details on sensor placement and data gathering are presented in Section \ref{sec:dataGathering}. Figures \ref{fig:ableAvatar} and \ref{fig:prosthesisAvatar} show the VRE avatars for the able-bodied and prosthetic cases. During the Training block of the experiment subjects were instructed outside the VRE on how to use the prosthetic interface and were allowed to familiarise themselves with it. This was done by presenting a third person view of the virtual residual limb and prosthetic device on a screen. The procedure was approved by the University of Melbourne Human Research Ethics Committee, project number 1750711.1. Informed consent was received from all subjects in the study. A video of the experimetal platform can be found in \textbf{ADD VIDEO OF EXPERIMENT}.

%
% Describe the protocol
%
\subsection{Data Gathering and Evaluation}
\label{sec:dataGathering}
Upper-body, arm, and hand position and orientation in 3D space was gathered using motion trackers. Muscle activation, used for the EP modality, was gathered using surface EMG electrodes. A summary of sensor type, location, and modalities where they were used are presented in Table \ref{ta:sensorInfo}. sEMG electrodes were placed on the forearm as the elbow brace interfered with the biceps/triceps eletrode placement used by transhumeral amputees. Furthermore, it was found that able-bodied subjects had a difficulty isolating biceps and triceps activation, which is required for the effective use of the EP modality. While this electrode position does not reflect the physiological placement of sEMG sensors for transhumeral prostheses, it can provide comparable functional capabilities.

%
% Sensor placement table
%
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Sensor placement and information.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Location & Sensor type & Reference frame & Modalities \\
        \hline
        \hline
        C7 Vertebra &  Motion  & Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Shoulder &  Motion  &  Virtual world (position)  &  All \\
        acromion &          & Sensor (orientation)      & \\
        \hline
        Upper-arm &  Motion &  Virtual world (position)  &  All \\
                    &          & Sensor (orientation)      & \\
        \hline
        Lower-arm &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Hand    &  Motion &  Virtual world (position)  &  AB \\
                &          & Sensor (orientation)      & \\
        \hline
        Forearm   &  sEMG &  -  &  EP \\
                  &       &     & \\
        \hline
    \end{tabular}
    \label{ta:sensorInfo}
    %\vspace{-5mm}
\end{table}

Three categories of metrics are used in this paper to evaluate the subject's performance of the task and the effects of prosthetic interfaces on the following aspects of reaching motion: task performance, quality of motion, and motor behaviour.
%
% Task
%
\subsubsection{Task Performance Metrics}
Two metrics of task performance are considered in this paper: completion time and reach accuracy.
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item \textit{Task completion time ($t_f^{\mu}$):} The mean task time over iterations of the task is used to determine the effects of prosthetic interfaces on the time required to complete the task. As this metric is commonly used in the literature, it is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature.
    \item \textit{Accuracy ($\delta^{\mu}$):} The mean reach accuracy over iterations of the task is used to verify that the task is being performed adequately.
\end{enumerate}

%
% Quality of motion
%
\subsubsection{Quality of Motion Metrics}
Two metrics of quality of motion are considered in this paper: path smoothness and variability.
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item \textit{Path smoothness ($\eta$):} Continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL) is used as the metric for smoothness \cite{Balasubramanian2012a} due to its characteristics which include sensitivity to changes in motor characteristics, robustness to measurement noise, and dimensionless monotonic response.
    \item \textit{Path variability ($\sigma_{\mu}$): } Low path variability, both of the hand and joints, is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint) is used as the metric for path variability.
\end{enumerate}

%
% Motor behaviour
%
\subsubsection{Motor Behaviour Metrics}
Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion. The metrics used in this paper use individual able-bodied motion as the point of reference for each subject. To provide a deeper analysis of motor behaviour, particularly with respect to movement patterns, individual behaviour will also be analysed in the results section in addition to the metrics presented next.
\begin{enumerate}[label=\textit{(\roman{*})}, wide, labelwidth=!, labelindent=0pt]
    \item \textit{Path difference ($\Delta_{\mu}$):} This metric evaluates the difference between the mean able-bodied hand/joint path and the mean prosthetic hand/joint path. This is used to determine the closeness of the resultant prosthetic motor behaviour to the individual's natural able-bodied motor behaviour. Let the mean hand/joint path for the able-bodied case ($AB$) be given by $\xv_{AB}^{\mu}(t_s n)$ and the mean path for the prosthetic case ($PC$) given by $\xv_{PC}^{\mu}(t_s n)$. The path difference ($\Delta_{\mu}$) is defined as the mean absolute difference between the mean paths across the time domain as follows.

    \begin{equation}
    \label{eq:handDiff}
        \Delta_{\mu} =  \sum_{n=0}^{N}\frac{\| \xv_{AB}^{\mu}(t_s n)- \xv_{PC}^{\mu}(t_s n) \|_2}{N}.
    \end{equation}
    
    \item \textit{Upper-body displacement ($\phi^{\mu}$):} This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Some level of upper-body motion is also part of natural able-bodied motion during reaching tasks.
\end{enumerate}

\subsection{Hardware Set-up}
The experiment was performed on an HTC Vive Pro HMD with the application developed in Unity3D. The experimental platform runs on an Intel Core i7-8700K processor at 3.7GHz, with 32GB RAM, and an Gigabyte GeForce GTX 1080Ti video card with 11GB GDDR5. HTC Vive Trackers were used for motion tracking, except for hand motion tracking where an HTC Vive Controller was used (HTC Vive system tracking capabilities can be found in \cite{Niehorster2017}). The Vive Trackers were attached directly to the subject's body using medical tape. Data gathering, and VR update were performed at 90Hz. Myoware sensors were used for sEMG data gathering with Ag-AgCl electrodes. The application used for the experiment can be downloaded from https://github.com/Rigaro/VRProEP.

==> old/5_methodology_v3.tex <==
%
% Experimental methodology
%
\section{Experimental Methodology}
% \begin{itemize}
%     \item Experiment was designed to analyse the performance of the proposed task-space synergy method and compare it with able-bodied behaviour, traditional sEMG-based prosthetic interfaces, and joint-space synergy-based prosthetic interfaces.
%     \item The experiment was performed in a VRE with able-bodied subjects as it allowed to gather both able-bodied and prosthetic motor behaviour data from the same subjects through virtual amputation and prosthetic fitting.
% \end{itemize}
An experiment was designed to analyse the performance of the proposed task-space synergy method when used in a basic prosthetic elbow. The resultant behaviour with the proposed task-space synergy-based prosthetic interface was compared with able-bodied behaviour, a traditional sEMG-based prosthetic interface, and a basic joint-space synergy-based prosthetic interface. The experiment was performed in a Head Mounted Display-based (HMD) Virtual Reality Environment (VRE) on able-bodied subjects. This allowed to gather both able-bodied and prosthetic motor behaviour data from the same subjects through virtual amputation and prosthetic fitting.

%
% Experiment set-up Figure
%
\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.29\textwidth}
    \includegraphics[width=\textwidth]{Figures/TaskPOVAnnotated.png}
    \caption{Side view of the task. The object start position and target locations were normalised to the subject's height and arm length.}
    \label{fig:sideView}
\end{subfigure}
~
\begin{subfigure}[t]{0.305\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectPOVAnnotated.png}
    \caption{Subject point of view of the task. Only one target location was presented per repetition of the task. Subjects were required to place the virtual hand on the orange circle before each repetition of the task.}
    \label{fig:subjectView}
\end{subfigure}

\begin{subfigure}[t]{0.30\textwidth}
    \includegraphics[width=\textwidth]{Figures/SubjectAnnotated.png}
    \caption{Subject with motion tracking sensors, elbow brace, and VR headset. Motion tracking sensors were placed on: C7 vertebrae, shoulder acromion, upper arm, forearm, and hand. An elbow immobiliser was used for the virtual prosthetic cases. In the EMG case, two sEMG sensors were placed on the subject's forearm.}
    \label{fig:subject}
\end{subfigure} 
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/AbleAvatarAnnotated.png}
    \caption{Able-bodied VR avatar. Motion trackers determine the motion of the forearm and hand avatars and the white markers. The elbow immobiliser was inactive to allow the subject to perform the task naturally.}
    \label{fig:ableAvatar}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{Figures/ProstheticAvatarAnnotated.png}
    \caption{Prosthetic VR avatar. The upper arm motion tracker was used to create a ``residual limb'' avatar to which the virtual prosthesis was attached. The rest of the trackers were presented only as white markers. The elbow immobiliser was engaged, and forearm and hand tracking was disabled.}
    \label{fig:prosthesisAvatar}
\end{subfigure}
\caption{Experimental platform and task set-up. (a) presents the side view of the task while (b) the subject point of view in VR. (c) presents motion tracking sensor placement. (d) and (e) present the virtual avatars for the able-bodied and prosthetic cases.}
\label{fig:taskSetup}
\end{figure*}
%
% Figure END
%

\subsection{Experiment Task and Set-up}
The task required subjects to pick and place an object in 3D space in the forward direction from a standing position in a VRE. Subjects were not allowed to step to perform the reaching task. An iteration of the task was considered from when the object was grasped until the object was placed. One object start position and four target positions were used. Start and target positions were normalised to each subject's height ($h$) and arm length ($\ell$). The target location details are presented in Table \ref{ta:targets}. Figure \ref{fig:sideView} shows the start and target locations in the VRE from a side view, while Figure \ref{fig:subjectView} shows them from a subject point of view.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Object start and target positions.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|p{3.8cm}|}
        \hline
        Target & $x (m)$ & $y (m)$ & $z (m)$ & Comment \\
        \hline
        \hline
        Start  &     $0.5\ell$     &     $0.5h$   &  0 & Reachable from a neutral, relaxed position with the upper-arm down and elbow bent $90\deg$.\\
        \hline
        Close  &     $0.75\ell$    &     $0.65h$   &  0.12 & Reachable with upper-body motion only.  \\
        \hline
        Mid  &     $1.0\ell$      &     $0.65h$   &  -0.12 & Reachable with either upper-body motion or arm extension only. \\
        \hline
        Far  &     $1.5\ell$      &     $0.65h$   &  0 & Reachable with both upper-body motion and arm extension only.  \\
        \hline
        High  &     $1.0\ell$      &     $0.9h$   &  0  & Reachable with both upper-body motion and arm extension only. \\
        \hline
    \end{tabular}
    \label{ta:targets}
    %\vspace{-5mm}
\end{table}

Four different experiment modalities were used, one able-bodied and three transhumeral prosthetic. 1) The able-bodied (AB) modality was used to determine the benchmark motor behaviour and task performance for each subject. 2) A standard dual-site differential surface EMG proportional prosthetic interface (EP) to command the prosthetic elbow's joint velocity \cite{Fougner2012} was used as the traditional prosthetic interface modality for comparison. 3) The proposed task-space synergy (TS) method (\ref{eq:taskSpaceSynergy}). 4) A Joint-space synergy method (JS) given by a shoulder-elbow flexion synergy was used as the synergistic prosthetic interface modality for comparison. The JS was given by $\dot{q}_e = \theta \dot{q}_s$; where $\dot{q}_e$ is the prosthetic elbow velocity, $\dot{q}_s$ the shoulder extension velocity, and $\theta = 1$ the synergy parameter calibrated for forward reaching tasks. Another set of JS data was gathered from representative subjects with an un-calibrated synergy ($\theta = 0.6$) in order to compare with the proposed TS method which does not require calibration outside of the measurement of the subject's arm.

Subjects were fitted with an elbow orthosis with motion tracking sensors attached to it, which allowed to immobilise the elbow in the prosthetic cases; as well as motion tracking sensors on the C7 vertebrae (trunk motion), the shoulder acromion (shoulder motion), and the hand (see Figure \ref{fig:subject}). In the AB case, motion of the upper-body, the whole arm and hand was directly mapped to the VRE through a virtual avatar as shown in Figure \ref{fig:ableAvatar}. In the prosthetic cases, transhumeral amputation was emulated in able-bodied subjects in the VRE by using the data from the upper-arm motion tracker to determine the motion of the virtual residual limb. A virtual prosthetic elbow, forearm, and hand were attached to the virtual residual limb as seen in Figure \ref{fig:prosthesisAvatar}. Only the virtual prosthetic elbow was actuated, while the forearm and hand were fixed.

Muscle activation, used for the EP modality, was gathered using sEMG electrodes. sEMG electrodes were placed on the forearm as the elbow orthosis interfered with the biceps/triceps electrode placement typically used in transhumeral amputees. Furthermore, it was found that able-bodied subjects had difficulty isolating biceps and triceps activation, which is required for the effective use of the EP modality. While the forearm electrode position does not reflect the physiological placement of sEMG sensors for transhumeral prostheses, it can provide comparable functional capabilities.

The following prosthetic interface simplifications were done in order to reduce the cognitive load on the subjects and to focus the experiment on the motor behaviour aspect of prosthesis use. 1) The functionality of the prosthetic elbow was enabled with a button press instead of relying on complex sEMG switching commands, such as co-contraction, which are common place in prosthetics and are a major issue with active prostheses to date \cite{Biddiss2007a}. 2) Grasping and releasing of the object were done automatically when the subject stopped moving the hand and was touching the object (grasp) or within the target area (release). This avoided the need to switch between elbow and hand control.

\subsection{Hardware Set-up}
The experiment was performed on an HTC Vive Pro HMD with the application developed in Unity3D. The experimental platform runs on an Intel Core i7-8700K processor at 3.7GHz, with 32GB RAM, and an Gigabyte GeForce GTX 1080Ti video card with 11GB GDDR5. HTC Vive Trackers were used for motion tracking, except for hand motion tracking where an HTC Vive Controller was used (HTC Vive system tracking capabilities can be found in \cite{Niehorster2017}). The C7 and shoulder acromion Vive Trackers were attached directly to the subject's body using medical tape. Data gathering, and VR update were performed at 90Hz. Myoware sensors were used for sEMG data gathering with Ag-AgCl electrodes. The application used for the experiment can be downloaded from https://github.com/Rigaro/VRProEP.

\subsection{Experimental Protocol}
The experiment was performed on 15 able-bodied subjects, six female and nine male. The age range was $[22, 34]$ and the median age $28$ years old. The experiment was performed in two different sessions lasting two hours each. Each session was done on different days, not more than a week apart. Each session tested two different modalities. The first modality tested for all subjects was AB which was used as the benchmark for individual motor behaviour. The following modalities (prosthetic-based) were randomly selected to minimise the bias introduced by the effects of learning on the data gathered. The sessions' procedure is presented in Table \ref{ta:protocol}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Experiment session protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|}
        \hline
        Step & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Introduction   &     5     &     No-VR \\
        \hline
        Sensor placement   &     15   &     No-VR    \\
        \hline
        Modality 1  &     50      &     VR  \\
        \hline
        Break   &     5      &     No-VR  \\
        \hline
        Modality 2  &     50      &     VR  \\
        \hline
    \end{tabular}
    \label{ta:protocol}
    %\vspace{-5mm}
\end{table}

Each block of modality testing consisted of 120 iterations of the task separated into three sets of 40 iterations. The procedure for each modality testing is presented in Table \ref{ta:modalityProtocol}. During the Training block of the experiment subjects were instructed outside the VRE on how to use the prosthetic interface and were allowed to familiarise themselves with it. This was done by presenting a third person view of the virtual residual limb and prosthetic device on a screen. The procedure was approved by the University of Melbourne Human Research Ethics Committee, project number 1750711.1. Informed consent was received from all subjects in the study. A video of the experimetal platform can be found in \textbf{ADD VIDEO OF EXPERIMENT}.
\begin{table}[ht]
%\vspace{-3mm}
    \caption{Modality testing block protocol.}
    %\vspace{-2mm}
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        Step & Task iterations per target & Time (minutes) & VR/No-VR \\
        \hline
        \hline
        Training   &     -    &     5    &     No-VR \\
        \hline
        Practice   &     5    &     -    &     VR    \\
        \hline
        Set 1      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 2      &     10   &     -   &     VR  \\
        \hline
        Break   &     -      &     1    &     VR  \\
        \hline
        Set 3      &     10   &     -   &     VR  \\
        \hline
    \end{tabular}
    \label{ta:modalityProtocol}
    %\vspace{-5mm}
\end{table}

\subsection{Data Gathering and Analysis}
The data gathered from motion tracking sensors and the VRE was used to analyse the performance of the subjects in terms of the task, quality of motion, and motor behaviour. Only the last set of 40 iterations for each modality was used for data analysis in order to reduce the effects of motor learning on the results. The metrics used for data analysis are presented next.

Two metrics of task performance are considered in this paper: completion time and reach accuracy. The mean task completion time ($t_f^{\mu}$) over iterations of the task is used to determine the effects of prosthetic interfaces on the time required to complete the task. As this metric is commonly used in the literature, it is used to compare the performance of the synergistic interfaces in this paper to other studies in the literature. The mean reach accuracy ($\delta^{\mu}$) over iterations of the task is used to verify that the task is being performed adequately.

Two metrics of quality of motion are considered in this paper: path smoothness and variability. Continuous, well coordinated movements are characteristic of trained and healthy motor behaviour. Hand and joint path smoothness are well documented and accepted measures of the quality of upper-limb motion \cite{Kistemaker2014, Balasubramanian2012b, DeLosReyes-Guzman2014}. Here Spectral Arc Length (SAL), represented by ($\eta$), is used as the metric for smoothness \cite{Balasubramanian2012a} due to its characteristics which include sensitivity to changes in motor characteristics, robustness to measurement noise, and dimensionless monotonic response. Low path variability, both of the hand and joints, is characteristic of trained and healthy motor behaviour \cite{Balasubramanian2012b, Darling1987}. Here the standard deviation of the path (hand or joint), represented by ($\sigma_{\mu}$), is used as the metric for path variability.

Motor behaviour, particularly movement patterns, is more difficult to quantify due to the person-to-person variations in motion. The metrics used in this paper use individual able-bodied motion as the point of reference for each subject. To provide a deeper analysis of motor behaviour, particularly with respect to movement patterns, individual behaviour will also be analysed in the results section in addition to the two metrics presented next. The first metric of motor behaviour is path difference ($\Delta_{\mu}$). This metric evaluates the difference between the mean able-bodied hand/joint path and the mean prosthetic hand/joint path. This is used to determine the closeness of the resultant prosthetic motor behaviour to the individual's natural able-bodied motor behaviour. Let the mean hand/joint path for the able-bodied case ($AB$) be given by $\xv_{AB}^{\mu}(t_s n)$ and the mean path for the prosthetic case ($PC$) given by $\xv_{PC}^{\mu}(t_s n)$. The path difference ($\Delta_{\mu}$) is defined as the mean absolute difference between the mean paths across the time domain as follows.

\begin{equation}
\label{eq:handDiff}
    \Delta_{\mu} =  \sum_{n=0}^{N}\frac{\| \xv_{AB}^{\mu}(t_s n)- \xv_{PC}^{\mu}(t_s n) \|_2}{N}.
\end{equation}
    
The second metric of motor behaviour is upper-body displacement ($\phi^{\mu}$). This metric evaluates the amount of upper-body motion used for the task. When a prosthetic device is not used effectively or is not adequate for the task this metric represents compensation motion. Some level of upper-body motion is also part of natural able-bodied motion during reaching tasks.

==> old/6_results.tex <==
%
% Experiment results
%
\section{Results}
Given that target locations were personalised to each subject, hand paths for all modalities and targets were normalised to the subject's arm length for their analysis similarly to \cite{Yang2002}. The results data-set (raw and processed) can be downloaded from \textbf{ADD GITHUB LINK}. The results are presented next.
%
% Task
%
\subsection{Task Performance Metrics}
%
% Time
%
\subsubsection{Task completion time ($t_f^{\mu}$)}
Results for task completion time are presented in Figure \ref{fig:time}, where the mean task completion time for the experiment population is presented for each modality and target. Synergistic interfaces on average had a 20\% shorter task completion time than sEMG for the Far target, which requires more complex coordinated motion (upper-body and upper-arm). This suggests that when EP can be used effectively and there is no sequential switching between the joints in the prosthetic limb, it can be as effective as synergistic interfaces. In \cite{Alshammary2018} it was shown that there was a significant reduction in task completion time with JS assisted EP; however, the study could not identify whether this was due to the motion activated elbow/hand sEMG switching or the synergistic interface itself. The results presented herein along with those presented in \cite{Alshammary2018} suggest that synergistic interfaces may prove to be most effective in multi-degree of freedom prostheses and complex tasks as expected.
%
% Accuracy
%
\subsubsection{Accuracy ($\delta^{\mu}$)}
Results for reach accuracy are presented in Figure \ref{fig:accuracy}, where the mean reach accuracy for the experiment population is presented for each modality and target. The results show that subjects were capable of performing the task with similar accuracy for all modalities and targets.

\begin{figure*}[ht]
\centering
    %
    % Reach time
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/01_TaskTime.eps}
        \caption{Population task completion time mean and standard deviation.}
        \label{fig:time}
    \end{subfigure}
    ~
    %
    % Accuracy
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/02_Accuracy.eps}
        \caption{Population reach accuracy mean and standard deviation.}
        \label{fig:accuracy}
    \end{subfigure}
    ~
    %
    % Hand smoothness
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/03_HandSAL.eps}
        \caption{Population hand path smoothness mean and standard deviation. The less negative the smoother the path.}
        \label{fig:handSAL}
    \end{subfigure}


    %
    % Joint smoothness
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/04_JointSAL.eps}
        \caption{Population joint path smoothness mean and standard deviation. The less negative the smoother the path.}
        \label{fig:jointSAL}
    \end{subfigure}
    ~
    %
    % Hand STD
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/05_HandPathVar.eps}
        \caption{Population hand path variability mean and standard deviation.}
        \label{fig:handVar}
    \end{subfigure}
    ~
    %
    % Joint STD
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/05_2_JointPathVar.eps}
        \caption{Population joint path variability mean and standard deviation.}
        \label{fig:jointVar}
    \end{subfigure}
    %
\caption{Experimental results for the Task Performance and Quality of Motion metrics.}
\label{fig:results1}
\end{figure*}
%
% Quality of motion
%
\subsection{Quality of Motion Metrics}
%
% Hand smoothness
%
\subsubsection{Hand path smoothness ($\eta_v$)}
Results for hand smoothness are presented in Figure \ref{fig:handSAL}, where the mean hand path spectral arc length for the experiment population is presented for each modality and target. A less negative value means a smoother path. It is important to highlight that this metric can be affected if the subject chose to not use, or to pre-position, the prosthetic device during a trial. This is because a movement that only includes the ``healthy'' joints of the subject will be inherently smooth. This can be clearly seen in the Close and High targets, as EP was mostly used to pre-position the prosthetic device before initiating the reaching movement. On the other hand, in the Far target, which required use of both upper-body motion and arm extension, the JS interface shows a 10\% improvement in smoothness for the Far target with respect to the EP and TS interfaces.

%
% Joint smoothness
%
\subsubsection{Joint path smoothness ($\eta_q$)}
Results for joint smoothness are presented in Figure \ref{fig:jointSAL}, where the mean joints path spectral arc length for the experiment population is presented for each modality and target. A less negative value means a smoother path. In this instance the JS modality shows an improvement over the other prosthetic interfaces for the Mid, Far, and High targets. The joint motion was 18\%, 24\%, and 15\% smoother than EP for the Mid, Far, and High targets respectively. On the other hand, the TS modality only shows a 17\% improvement in joint smoothness for the Far target with respect to EP.

%
% Hand path variation
%
\subsubsection{Standard deviation of the hand trajectory ($\sigma_{\mu, p}$)}
Results for hand path variability are presented in Figure \ref{fig:handVar}, where the mean hand path standard deviation for the experiment population is presented for each modality and target. In this case the synergistic interfaces show lower hand path variability over EP for the Far target, with TS showing a 16\% reduction in variability over EP, and JS a 31\% reduction over EP.

%
% Joint path variation
%
\subsubsection{Standard deviation of the joints trajectory ($\sigma_{\mu, q}$)}
Results for joint path variability are presented in Figure \ref{fig:jointVar}, where the mean joint path standard deviation for the experiment population is presented for each modality and target. The synergistic interfaces show lower joint path variability over EP for the Far and High targets; however, EP and TS show high inter-subject variability for the High target. For the Far target case TS shows a 20\% reduction in joint path variability over EP while JS a 31\% reduction over EP.

%
% Motor behaviour
%
\subsection{Motor Behaviour Metrics}
%
% Hand path difference
%
\subsubsection{Hand path difference ($\Delta_{\mu, p}$)}
Results for hand path difference are presented in Figure \ref{fig:handDiff}, where the mean difference between the able-bodied hand path and the prosthetic modalities hand path for the experiment population is presented for each prosthetic modality and target. The JS modality shows an improvement over the other prosthetic interfaces for the Far target, being 24\% closer to the able-bodied hand path than EP and TS. This suggests that for complex coordinated movements the JS interface may be able to render the more natural hand path. Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}, these will be discussed in more detail in Section \ref{sec:handPathAnalysis}. 

\begin{figure*}[ht]
\centering
    %
    % Hand diff
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/07_HandPathDifference.eps}
        \caption{Population hand path difference mean and standard deviation.}
        \label{fig:handDiff}
    \end{subfigure}
    ~
    %
    % Joint diff
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/08_JointPathDifference.eps}
        \caption{Population joint path difference mean and standard deviation.}
        \label{fig:jointDiff}
    \end{subfigure}
    
    %
    % C7 displacement
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=1.1\textwidth]{Figures/Results/06_1_C7Displacement.eps}
        \caption{Population C7 displacement mean and standard deviation.}
        \label{fig:C7Displacement}
    \end{subfigure}
    ~
      %(or a blank line to force the subfigure onto a new line)
    % Shoulder displacement
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=1.1\textwidth]{Figures/Results/06_2_SADisplacement.eps}
        \caption{Population shoulder acromion displacement mean and standard deviation.}
        \label{fig:SADisplacement}
    \end{subfigure}
        %
\caption{Experimental results for the Motor Behaviour metrics.}
\label{fig:results2}
\end{figure*}

%
% Joints relationship difference
%
\subsubsection{Joints relationship difference ($\Delta_{\mu, q}$)}
Results for joints relationship difference are presented in Figure \ref{fig:jointDiff}, where the mean difference between the able-bodied joints relationship and the prosthetic modalities joints relationship for the experiment population is presented for each prosthetic modality and target. The JS modality shows an improvement over the other prosthetic interfaces for the Close and Far targets. JS is 28\% closer to able-bodied joint behaviour than EP and TS for the Close target, and 19\% and 35\% closer than EP and TS to able-bodied joint behaviour for the Far target. The result for the Far target suggests that for complex coordinated movements the JS interface may be able to render the more natural motor behaviour. It is important to note that there is a high degree of inter-subject variability for the EP modality while TS and JS show lower variability. This suggests that subjects were consistently capable of effectively using the synergistic interfaces, unlike with EP where some subjects may not have been able to use it effectively. This highlights the intuitiveness of synergistic interfaces, which suggests that they may be easier to learn. Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}, these will be discussed in more detail in Section \ref{sec:jointSynergyAnalysis}.

%
% Upper-body displacement
%
\subsubsection{Upper-body displacement ($\phi_{\mu}$)}
Results for upper-body displacement are presented in Figure \ref{fig:results2}, where the mean C7 and shoulder acromion displacement for the experiment population are presented in Figures \ref{fig:C7Displacement} and \ref{fig:SADisplacement}, respectively, for each modality and target. These results show that subjects performed the task with similar upper-body displacement across all modalities, meaning that they purposely used the prosthetic device as much as possible to perform the task as instructed. As such, the effects of prosthetic interfaces on motor behaviour in this study are better determined by the trajectories rather than the resultant upper-body displacement.

%
% Motion patterns analysis
%
\subsection{Motion Patterns Analysis}
Given that the more significant motor behaviour changes are observed for the Far target, the motion pattern analysis will focus on the results for such target.

\subsubsection{Hand path}
\label{sec:handPathAnalysis}
Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}. The normalised AB hand path follows the shape typically seen in reaching movements \cite{Yang2002}, this shows that the VRE did not affect the motor behaviour of subjects. While some subjects were not able of achieving able-bodied-like hand motion with any type of prosthetic interface within the time allowed for the experiment, some interesting patterns can be observed in these results. As expected from the EP case, the hand follows a more irregular path as the user manually adjusts the elbow position throughout the reaching motion. 

In the case of the TS interface, the two step movement strategy required by it can seen in the results for subjects 8, 12, and 14. The strategy involves an initial hand pre-position movement characterised by a smooth upward/forward hand movement, followed by a mostly straight hand path due to the task-space synergy. While this behaviour was also observed in the task iteration results of the other subjects, these do not appear in the mean hand path due to averaging effects. It should also be noted that subjects 3, 6, and 11 were capable of achieving on average a TS hand path nearly identical to their AB. This suggests that these subjects found a way to utilise the interface to achieve the most natural hand path.

On the other hand, a larger number of subjects were capable of achieving nearly overlapping AB hand path with the JS interface, subjects 2, 3, 5, 6, 10, and 14. This suggests that JS may be easier to learn due to its reduced complexity.  These differences are captured by the metrics related to hand quality of motion and behaviour $\eta_v$, $\sigma_{\mu,p}$, and $\Delta_{\mu,p}$, where JS performed better than TS.
%
% Figure
%
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/Results/09_HandFunnels.eps}
    \caption{Mean hand path for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green.}
    \label{fig:handFunnels}
\end{figure*}


\subsubsection{Shoulder-elbow flexion relationship}
\label{sec:jointSynergyAnalysis}
Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}. It is important to highlight that this could be seen as the natural shoulder-elbow flexion synergy for the AB case. This AB shoulder-elbow relationship is characterised for being a smooth curve. On the other hand, EP is composed of two mostly straight lines, one horizontal and one vertical (or with high slope). These correspond to mostly sequential shoulder and elbow motion. This behaviour is commonly seen with this type of prosthetic interface. 

TS is composed of a straight horizontal line and a smooth curve. These correspond to the initial pre-positioning of the hand followed by a coordinated movement. Given that the interface was designed to operate in such way due to the lack of information (target position), this resultant behaviour is expected. This highlights how the interface design can directly affect the motor behaviour of prosthesis users and should be taken in consideration when designing prosthetic interfaces. JS is composed of a smooth curve in most subjects, pointing towards a mostly coordinated movement. This is an interesting result as it suggests that the subjects learned to use the synergy enabling mechanism (button press) to activate the elbow such that the most natural reaching motion possible was performed. 

Lastly, in some subjects it is possible to observe a short shoulder only movement at the end of the reach for both TS and JS cases (e.g. subject 4). This appears as a result of having to compensate for an inaccurate initial reach, which then needed to be corrected while the elbow was fixed in position as it would otherwise result in elbow flexion. These differences in motor behaviour between TS and JS are captured by the joint path smoothness ($\eta_{\mu,q}$) and difference metrics ($\Delta_{\mu,q}$), where JS performed better than TS.
%
% Figure
%
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/Results/10_JointFunnels.eps}
    \caption{Mean shoulder-elbow flexion relationship for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green. The origin represents the arm extended forward.}
    \label{fig:jointFunnels}
\end{figure*}

==> old/6_results_v2.tex <==
%
% Experiment results
%
% Percentage: ((T - A) - (E - A)) / (E - A)
\section{Results}
Given that target locations were personalised to each subject, hand paths for all modalities and targets were normalised to the subject's arm length for their analysis similarly to \cite{Yang2002}. The results data-set (raw and processed) can be downloaded from \textbf{ADD GITHUB LINK}. The results are presented next.

\begin{figure*}[hb]
\centering
    %
    % Reach time
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/01_TaskTime.eps}
        \caption{Population task completion time mean and standard deviation.}
        \label{fig:time}
    \end{subfigure}
    ~
    %
    % Accuracy
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/02_Accuracy.eps}
        \caption{Population reach accuracy mean and standard deviation.}
        \label{fig:accuracy}
    \end{subfigure}
    ~
    %
    % Hand smoothness
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/03_HandSAL.eps}
        \caption{Population hand path smoothness mean and standard deviation. The less negative the smoother the path.}
        \label{fig:handSAL}
    \end{subfigure}


    %
    % Joint smoothness
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/04_JointSAL.eps}
        \caption{Population joint path smoothness mean and standard deviation. The less negative the smoother the path.}
        \label{fig:jointSAL}
    \end{subfigure}
    ~
    %
    % Hand STD
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/05_HandPathVar.eps}
        \caption{Population hand path variability mean and standard deviation.}
        \label{fig:handVar}
    \end{subfigure}
    ~
    %
    % Joint STD
    \begin{subfigure}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/05_2_JointPathVar.eps}
        \caption{Population joint path variability mean and standard deviation.}
        \label{fig:jointVar}
    \end{subfigure}
    %
\caption{Experimental results for the Task Performance and Quality of Motion metrics.}
\label{fig:results1}
\end{figure*}
%
% Task
%
\subsection{Task Performance Metrics}
%
% Time
%
\subsubsection{Task completion time ($t_f^{\mu}$)}
Results for task completion time are presented in Figure \ref{fig:time}, where the mean task completion time for the experiment population is presented for each modality and target. Synergistic interfaces on average had a 20\% shorter task completion time than sEMG for the Far target, which requires more complex coordinated motion (upper-body and upper-arm), with both TS and JS performing similarly. This suggests that TS is as effective as JS in reducing the time required to perform reaching tasks.
%
% Accuracy
%
\subsubsection{Accuracy ($\delta^{\mu}$)}
Results for reach accuracy are presented in Figure \ref{fig:accuracy}, where the mean reach accuracy for the experiment population is presented for each modality and target. The results show that subjects were capable of performing the task with similar accuracy for all modalities and targets.
%
% Quality of motion
%
\subsection{Quality of Motion Metrics}
%
% Hand smoothness
%
\subsubsection{Hand path smoothness ($\eta_v$)}
Results for hand smoothness are presented in Figure \ref{fig:handSAL}, where the mean hand path spectral arc length for the experiment population is presented for each modality and target. A less negative value means a smoother path. It is important to highlight that this metric can be affected if the subject chose to not use, or to pre-position, the prosthetic device during a trial. This is because a movement that only includes the ``healthy'' joints of the subject will be inherently smooth. This can be clearly seen in the Close and High targets, as EP was mostly used to pre-position the prosthetic device before initiating the reaching movement. On the other hand, in the Far target, which required use of both upper-body motion and arm extension, the JS interface shows a 10\% improvement in smoothness for the Far target with respect to EP, while TS shows no improvement. This may be attributed to the need with TS to pre-position the hand before executing the movement, which affects the resultant SAL.

%
% Joint smoothness
%
\subsubsection{Joint path smoothness ($\eta_q$)}
Results for joint smoothness are presented in Figure \ref{fig:jointSAL}, where the mean joints path spectral arc length for the experiment population is presented for each modality and target. A less negative value means a smoother path. In this instance the JS modality shows an improvement over the other prosthetic interfaces for the Mid, Far, and High targets. The joint motion was 18\%, 24\%, and 15\% smoother than EP for the Mid, Far, and High targets respectively. On the other hand, the TS modality only shows a 17\% improvement in joint smoothness for the Far target with respect to EP. This metric is affected similarly to hand path smoothness.

%
% Hand path variation
%
\subsubsection{Standard deviation of the hand trajectory ($\sigma_{\mu, p}$)}
Results for hand path variability are presented in Figure \ref{fig:handVar}, where the mean hand path standard deviation for the experiment population is presented for each modality and target. In this case the synergistic interfaces show lower hand path variability over EP for the Far target, with TS showing a 16\% reduction in variability over EP, and JS a 31\% reduction over EP.

%
% Joint path variation
%
\subsubsection{Standard deviation of the joints trajectory ($\sigma_{\mu, q}$)}
Results for joint path variability are presented in Figure \ref{fig:jointVar}, where the mean joint path standard deviation for the experiment population is presented for each modality and target. The synergistic interfaces show lower joint path variability over EP for the Far and High targets; however, EP and TS show high inter-subject variability for the High target. For the Far target case TS shows a 20\% reduction in joint path variability over EP while JS a 31\% reduction over EP.

%
% Motor behaviour
%
\subsection{Motor Behaviour Metrics}
        %
%
% Hand path difference
%
\subsubsection{Hand path difference ($\Delta_{\mu, p}$)}
Results for hand path difference are presented in Figure \ref{fig:handDiff}, where the mean difference between the able-bodied hand path and the prosthetic modalities hand path for the experiment population is presented for each prosthetic modality and target. The JS modality shows an improvement over the other prosthetic interfaces for the Far target, being 24\% closer to the able-bodied hand path than EP, while TS shows no improvement. This may be attributed to TS' need to pre-position the hand before the reaching motion. Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}, these will be discussed in more detail in Section \ref{sec:handPathAnalysis}. 
%
% Joints relationship difference
%
\subsubsection{Joints relationship difference ($\Delta_{\mu, q}$)}
Results for joints relationship difference are presented in Figure \ref{fig:jointDiff}, where the mean difference between the able-bodied joints relationship and the prosthetic modalities joints relationship for the experiment population is presented for each prosthetic modality and target. The JS modality shows an improvement over the other prosthetic interfaces for the Close and Far targets. JS is 28\% closer to able-bodied joint behaviour than EP and TS for the Close target, and 19\% closer than EP to able-bodied joint behaviour for the Far target, while there is no improvement for the TS case. Again, this can be attributed to the pre-positioning movement. It is important to note that there is a high degree of inter-subject variability for the EP modality while TS and JS show lower variability. This suggests that subjects were consistently capable of effectively using the synergistic interfaces, unlike with EP where some subjects may not have been able to use it effectively. This highlights the intuitiveness of synergistic interfaces, which suggests that they may be easier to learn. Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}, these will be discussed in more detail in Section \ref{sec:jointSynergyAnalysis}.

\begin{figure}[ht]
\centering
    %
    % Hand diff
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/07_HandPathDifference.eps}
        \caption{Population hand path difference mean and standard deviation.}
        \label{fig:handDiff}
    \end{subfigure}
    ~
    %
    % Joint diff
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{Figures/Results/08_JointPathDifference.eps}
        \caption{Population joint path difference mean and standard deviation.}
        \label{fig:jointDiff}
    \end{subfigure}
\caption{Experimental results for the hand and joint path difference.}
\label{fig:results2}
\end{figure}


%
% Upper-body displacement
%
\subsubsection{Upper-body displacement ($\phi_{\mu}$)}
Results for mean C7 and shoulder acromion displacement for the experiment population are presented in Figures \ref{fig:C7Displacement} and \ref{fig:SADisplacement}, respectively, for each modality and target. C7 displacement for the TS case shows a 60\% and 45\% reduction over EP and JS, respectively, for the Mid target; while a 60\% reduction over EP and JS for the Far target. Shoulder acromion displacement for the TS case was the same as able-bodied for the Mid and Far targets.
    

%(or a blank line to force the subfigure onto a new line)
% Shoulder displacement
\begin{figure}[ht]
\centering
    %
    % C7 displacement
    \begin{subfigure}[t]{0.22\textwidth}
        \includegraphics[width=1.1\textwidth]{Figures/Results/06_1_C7Displacement_v2.eps}
        \caption{Population C7 displacement mean and standard deviation.}
        \label{fig:C7Displacement}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.22\textwidth}
    %\includegraphics[width=0.32\textwidth]{Figures/Results/06_2_SADisplacement.eps}
        \includegraphics[width=1.1\textwidth]{Figures/Results/06_2_SADisplacement_v2.eps}
        \caption{Population shoulder acromion displacement mean and standard deviation.}
        \label{fig:SADisplacement}
    \end{subfigure}
    \caption{Experimental results for the C7 and shoulder acromion displacement metrics.}
\end{figure}

%
% Motion patterns analysis
%
\subsection{Motion Patterns Analysis}
Given that the more significant motor behaviour changes are observed for the Far target, the motion pattern analysis will focus on the results for such target.

\subsubsection{Hand path}
\label{sec:handPathAnalysis}
Mean hand paths for each subject and modality for the Far target are presented in Figure \ref{fig:handFunnels}. The normalised AB hand path follows the shape typically seen in reaching movements \cite{Yang2002}, this shows that the VRE did not affect the motor behaviour of subjects. While some subjects were not able of achieving able-bodied-like hand motion with any type of prosthetic interface within the time allowed for the experiment, some interesting patterns can be observed in these results. As expected from the EP case, the hand follows a more irregular path as the user manually adjusts the elbow position throughout the reaching motion. 

In the case of the TS interface, the two step movement strategy required by it can seen in the results for subjects 8, 12, and 14. The strategy involves an initial hand pre-position movement characterised by a smooth upward/forward hand movement, followed by a mostly straight hand path due to the task-space synergy. While this behaviour was also observed in the task iteration results of the other subjects, these do not appear in the mean hand path due to averaging effects. It should also be noted that subjects 3, 6, and 11 were capable of achieving on average a TS hand path nearly identical to their AB. This suggests that these subjects found a way to utilise the interface to achieve the most natural hand path.

On the other hand, a larger number of subjects were capable of achieving nearly overlapping AB hand path with the JS interface, subjects 2, 3, 5, 6, 10, and 14. This suggests that JS may be easier to learn due to its reduced complexity.  These differences are captured by the metrics related to hand quality of motion and behaviour $\eta_v$, $\sigma_{\mu,p}$, and $\Delta_{\mu,p}$, where JS performed better than TS.
%
% Figure
%
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[t]{0.80\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{Figures/Results/09_HandFunnels.eps}
    \caption{Mean hand path for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green.}
    \label{fig:handFunnels}
    \end{subfigure}
    
    %
    % Figure
    %
    \begin{subfigure}[t]{0.80\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{Figures/Results/10_JointFunnels.eps}
    \caption{Mean shoulder-elbow flexion relationship for all subjects (S1-S15) for the Far Target. AB hand path presented in black, EP in blue, TS in red, and JS in green. The origin represents the arm extended forward.}
    \label{fig:jointFunnels}
    \end{subfigure}
    \caption{Experimental results for the hand and joint paths.}
\end{figure*}


\subsubsection{Shoulder-elbow flexion relationship}
\label{sec:jointSynergyAnalysis}
Mean joint relationships for each subject and modality for the Far target are presented in Figure \ref{fig:jointFunnels}. It is important to highlight that this could be seen as the natural shoulder-elbow flexion synergy for the AB case. This AB shoulder-elbow relationship is characterised for being a smooth curve. On the other hand, EP is composed of two mostly straight lines, one horizontal and one vertical (or with high slope). These correspond to mostly sequential shoulder and elbow motion. This behaviour is commonly seen with this type of prosthetic interface. 

TS is composed of a straight horizontal line and a smooth curve. These correspond to the initial pre-positioning of the hand followed by a coordinated movement. Given that the interface was designed to operate in such way due to the lack of information (target position), this resultant behaviour is expected. This highlights how the interface design can directly affect the motor behaviour of prosthesis users and should be taken in consideration when designing prosthetic interfaces. JS is composed of a smooth curve in most subjects, pointing towards a mostly coordinated movement. This is an interesting result as it suggests that the subjects learned to use the synergy enabling mechanism (button press) to activate the elbow such that the most natural reaching motion possible was performed. 

Lastly, in some subjects it is possible to observe a short shoulder only movement at the end of the reach for both TS and JS cases (e.g. subject 4). This appears as a result of having to compensate for an inaccurate initial reach, which then needed to be corrected while the elbow was fixed in position as it would otherwise result in elbow flexion. These differences in motor behaviour between TS and JS are captured by the joint path smoothness ($\eta_{\mu,q}$) and difference metrics ($\Delta_{\mu,q}$).

==> old/7_discussion.tex <==
%
% Discussion
%
\section{Discussion}
Synergistic interfaces allow the coordinated motion required for natural reaching motor behaviour. Subjects that became proficient with these interfaces within the time allowed for the experiment were able to achieve near-able-bodied movement patterns, showing the capabilities of synergistic interfaces. These results suggest that as subjects learned to use the device, they found that the most intuitive, or natural, way of using the prosthetic device was in a similar fashion to able-bodied movements. While JS are not explicitly designed for arbitrary point-to-point reaching tasks, subjects were able to determine the best way to use it in a natural way. Whether this was done consciously or subconsciously cannot be determined by the study herein; however, it is an interesting question that remains open for investigation. The subjects in the study were all able-bodied, so they were not affected by the changes in motor behaviour experienced by amputees. An important aspect to study is whether the same results are obtained with subjects who have used a prosthetic device for a long time, as their motor behaviour would have significantly changed.
    
In this study, compensation motion was observed to be comparable across all modalities, while other studies have found that compensation motion may be reduced through the use of synergistic interfaces \cite{Merad2018}. This may be caused by the difference in experimental design and instruction provided to the subjects. Here the hand start position was defined instead of the joint start position, and subjects were instructed to use the prosthetic device as much as possible. The authors acknowledge that if the subjects were to be left to figure out how to use the device by themselves this may result differently, as they may choose to use the device less due to the required cognitive load imposed by the interface. However, this may affect other metrics, such as task completion time, differently.
    
The results suggest that the synergy formulation does not significantly impact the outcome of the task or motor behaviour. While JS showed some advantages over TS, the difference was not significant. It appears that subjects were able to internally compensate for the two different mappings (joint-to-joint and joint-to-task), and so were able to use both synergistic interfaces effectively. TS, however, introduced an additional movement due to the lack of information (object location) available to generate the desired hand path, as such hampering its effectiveness. These interfaces appear to differ in their learning curve as well. JS was observed to be easier to use (joint-space to joint-space mapping) while TS was more difficult to use (joint-space to task-space mapping) as seen by the number of subjects that were able to achieve proficiency with the interface, as measured by the motor behaviour metrics. This suggests that the joint-to-task mapping may affect the complexity and intuitiveness of the interface. This could be mitigated by changing how the TS training is provided to the subjects. The study only considered short term motor adaptation, and changes in motor behaviour could appear over extended periods of use. Such longitudinal studies will be considered in the later stages of this research.

The joint-space synergy used in the study only provided a one-to-one relationship between shoulder and elbow flexion velocity. However, it has been found that personalising the JS interface to its user can improve its performance \cite{Legrand2018, Garcia-Rosas2019}. Therefore, it may be possible to further improve the performance of JS over EP and TS by personalising the interface. On the other hand, the simple prosthesis considered in the study may not highlight the advantages of a task-space synergy, as this type of synergy can provide simultaneous control of hand orientation as well; which is needed for richer tasks such as drinking. The additional degrees of freedom in the wrist add significant complexity to sEMG interfaces making them even more difficult to use, further motivating the use of synergies. This added complexity will be studied in future work.


==> old/7_discussion_v2.tex <==
%
% Discussion
%
\section{Discussion}
Synergistic interfaces allow the coordinated motion required for natural reaching motor behaviour. Subjects that became proficient with these interfaces within the time allowed for the experiment were able to achieve near-able-bodied movement patterns, showing the capabilities of synergistic interfaces. These results suggest that as subjects learned to use the device, they found that the most intuitive, or natural, way of using the prosthetic device was in a similar fashion to able-bodied movements. While JS are not explicitly designed for arbitrary point-to-point reaching tasks, subjects were able to determine the best way to use it in a natural way. Whether this was done consciously or subconsciously cannot be determined by the study herein; however, it is an interesting question that remains open for investigation. The subjects in the study were all able-bodied, so they were not affected by the changes in motor behaviour experienced by amputees. An important aspect to study is whether the same results are obtained with subjects who have used a prosthetic device for a long time, as their motor behaviour would have significantly changed.

The results suggest that the synergy formulation does not significantly impact the outcome of the task or motor behaviour, where both TS and JS showing overall improvements, TS reducing upper-body compensation motion, and JS resulting in smoother motion. It appears that subjects were able to internally compensate for the two different mappings (joint-to-joint and joint-to-task), and so were able to use both synergistic interfaces effectively. TS, however, introduced an additional movement due to the lack of information (object location) available to generate the desired hand path, as such hampering its effectiveness. These interfaces appear to differ in their learning curve as well. JS was observed to be easier to use (joint-space to joint-space mapping) while TS was more difficult to use (joint-space to task-space mapping) as seen by the number of subjects that were able to achieve proficiency with the interface, as measured by the motor behaviour metrics. This suggests that the joint-to-task mapping may affect the complexity and intuitiveness of the interface. This could be mitigated by changing how the TS training is provided to the subjects. Moreover, if complete information on the target is available, the pre-positioning movement would not be necessary, thus simplifying the interface. This case warrants investigation as task-space synergies have the potential to be generalisable to any reaching motion and are inherently personalised as a model of the user's arm is used in their formulation. 

Lastly, the simple virtual elbow prosthesis considered in the study may not highlight the advantages of a task-space synergy, as this type of synergy can provide simultaneous control of hand orientation as well; which is needed for richer tasks such as drinking. The additional degrees of freedom in the wrist add significant complexity to sEMG interfaces making them even more difficult to use, further motivating the use of synergies. This added complexity will be studied in future work.


==> old/8_conclusion.tex <==
%
% Discussion
%
\section{Conclusion}
In this paper a realisation of a task-space synergy for motion-based human-prosthetic interfaces was presented. This type of synergy allows the prosthesis to be controlled in task-space, i.e. to directly control the path of the prosthetic hand instead of its joints. Such type of synergistic interface may prove useful in complex tasks that require the coordination of multiple degrees of freedom. A study on the effects of two types of synergistic interfaces, joint-space and task-space, on task performance and motor behaviour was presented. The study was performed on 15 able-bodied subjects in a Virtual Reality Environment (VRE), where amputation was emulated through the motion reported to the VRE.

Results showed that the use of synergistic interfaces do indeed results in able-bodied-like motor behaviour in prosthesis users. While there was no significant difference between the performance of task-space and joint-space synergies, it was found that the design of the synergistic interface influenced the resultant motor behaviour. In the task-space synergy, the limited information on the task resulted in an additional step to motor planning, resulting in a larger difference to able-bodied motion than the joint-space synergy interface. Moreover, a larger number of subjects were able to learn to use the joint-space synergy interface effectively as shown by their able-bodied-like motor behaviour compared to the task-space type, suggesting that the simplicity of such interface may prove advantageous.

Future studies will investigate the performance of synergistic prosthetic interfaces in tasks with higher complexity and with multi-degree-of-freedom prosthetic devices, by introducing hand orientation to the task and a multi-articulated wrist to the prosthetic device. The performance of a more complex task-space synergy with such device will be evaluated. Lastly, the effects of personalisation of joint-space synergies on motor behaviour will be investigated.

==> old/_abstracts.tex <==

%Synergistic prostheses use motion of the residual-limb joints to determine the motion of the prosthetic joints, enabling coordination of the human-prosthetic arm as required by activities of daily living. These joint-space synergies are dependent on individual motor behaviour and the task, requiring personalisation and task calibration. Alternatively, a task-space synergy which is characterised by the arm kinematics (individuality) and the hand motion (task) could be employed. These synergies may be advantageous in prosthetics as the task and personalisation are explicit in their formulation, averting the need for task-dependent synergies and personalisation.
%This paper proposes a task-space synergy for upper-limb human-prosthetic interfaces, which takes a robotics approach to the challenge of arbitrary point-to-point forward reaching task by constraining and normalising the desired hand motion, and utilising voluntary information from the prosthesis user. 
%The proposed method is compared against traditional and synergistic prosthetic interfaces in a study of motor behaviour and task performance on able-bodied subjects using a virtual prosthetic elbow.
%Experimental results showed that for a set of forward reaching tasks the proposed task-space synergy achieves comparable performance to joint-space synergies in terms of the closeness to able-bodied-like motor behaviour and task performance without the need for personalisation or synergy calibration.%Synergistic prosthetic interfaces determine the motion of the prosthetic device as a function of the motion of the residual limb. This enables the coordinated human-prosthetic arm motion required by many activities of daily living. Typically, this relationship is done at a joint level; however, another possibility is to realise the relationship in task-space. Task-space synergies explicitly relate the motion of the residual limb to the hand path. These could have an advantage over joint-space synergies in terms of the resultant upper-limb motor behaviour, as it is theorised that human upper-limb motion planning is done in task-space. Regardless of the method used for the realisation of the synergistic prosthetic interface, their effects on motor behaviour are not widely understood due to the limited number of studies in the field to date. This paper presents a set of metrics to evaluate task performance, quality of motion, and motor behaviour in the context of synergistic prostheses. These metrics are then used in a study of quality of motion and movement patterns on able-bodied subjects using a virtual prosthetic elbow with different prosthetic interfaces (traditional and synergistic) in a Virtual Reality Environment. The study was aimed to determine how synergistic prosthetic interfaces, both in joint-space and task-space, perform in comparison to traditional prosthetic interfaces in terms of their capability to restore able-bodied motor behaviour. Given that task-space synergies are yet to be considered for transhumeral prosthetic applications, a novel method to realise these synergies in the context of the application is presented. Experimental results showed that the use of synergistic interfaces does result in able-bodied-like motor behaviour in emulated prosthesis users. While there was no significant difference between the performance of task-space and joint-space synergies, it was found that the design of the synergistic interface influenced the resultant motor behaviour.

==> old/older/1_intro_vTS.tex <==
%
% Introduction
%
\section{Introduction}
%
%

\begin{itemize}
    \item Introduce the challenge of performing ADLs with current prostheses.
\end{itemize}
%
% What is the main challenge that we are studying in this paper?
% Coordinated motion is required for ADLs.
% This is not possible with current prostheses.
%
The coordinated motion of the joints in the upper limb is required for most Activities of Daily Living (ADLs).
Carrying out these ADLs using current prosthetic devices is a challenge as these devices are only capable of sequential Degree of Freedom (DOF) motion \cite{Fougner2012}, i.e. one joint at a time. This is largely due to the limitations of the human-prosthetic interfaces (referred to as HPIs henceforth) available commercially \cite{Biddiss2007}.

\begin{itemize}
    \item Introduce synergies in prosthetics and advantages.
\end{itemize}   
%
% What is a possible solution for this challenge in the literature?
% A novel kinematic synergy based HPI allows for coordinated motion.
%
In the context of transhumeral prostheses, novel experimental HPIs, such as kinematic synergies and pattern recognition based interfaces \cite{Alshammary2018,Ortiz-Catalan2014}, have permitted the coordinated motion of the DOFs in a prosthesis with those of the residual limb. Particularly, kinematic synergies-based HPIs directly relate the motion of the residual limb with that of the prosthesis by using residual limb motion measurements rather than muscle contraction. Thus creating a ``Synergy'' between the human joints and prosthetic joints, which inherently allows for coordinated human-prosthesis arm motion.

\begin{itemize}
    \item Review of neural-network based synergies to highlight challenges with current methods.
\end{itemize}
%
% What are the limitations of this solution?
% Synergies are individual and task/path dependent.
%
Kinematic synergies, however, also have their limitations; mostly due to their observed dependency to human motor behaviour and preference, and the desired reaching motion, or task  \cite{Merad2018, Gottlieb1997, Garcia-Rosas2018EMBC}. These dependencies have also been shown to occur on able-bodied individuals \cite{Bockemuhl2010}. 
%
% What are possible solutions to these limitations in the literature?
% Personalization, our work.
% Task dependency is still an open question. Examples of how the synergy depends on start and end position. How it is possible to reach in 3D from a single start point.
%
%
% What do these lack?
% We know from traditional kinematic analysis that end effector path is a function of both the joints angular position and velocity. All current formulations only consider either one.
%
The kinematic synergies-based HPIs in the literature have been formulated as either a function of the angular position or velocity of the residual limb joints \cite{Alshammary2018, Legrand2018}, thus acting only in joint-space. Furthermore, most of the methods to generate the synergies require full arm motion data, typically gathered from able-bodied subjects \cite{Khalil2013, Legrand2018}; thus introducing its own set of challenges \cite{Merad2018}.
These synergies have only been considered for specific starting positions with the ability to reach multiple targets \cite{Legrand2018, Akhtar2017, Blana2016}, and it has been observed that the generated synergies depend on the pre-defined starting position. However, the challenge with reaching motion is that it is constituted of arbitrary start and end positions. While it has been found that arbitrary point-to-point hand path can be normalised \cite{Yang2002}, the challenge to generalise these synergies for any combination of start and end positions in the human arm workspace remains.


Review of EMG + Synergy with autonomous switching:
\begin{itemize}
    \item An attempt to address the challenge of reaching from-and-to arbitrary positions with a synergistic prosthetic elbow was presented in \cite{Alshammary2018}.
    \item A kinematic elbow synergy was combined with sEMG to control a virtual prosthetic elbow.
    \item A constant scalar synergy was chosen and was linearly combined with dual-site proportional sEMG.
    \item Furthermore, the virtual prosthesis included a hand such that the user had to switch between the elbow and the hand to perform a grasp-and-drop-off task.
    \item The proposed method, which also included IMU-based automated switching between elbow and hand, was compared against traditional dual-site proportional sEMG control with co-contraction switching.
    \item In the results it was observed that the time required to perform the task was significantly reduced while no change in compensation motion seen with the proposed method.
    \item However, it was not possible to discern whether the task time difference was due to the synergy component or the automated elbow-hand control switching.
\end{itemize}


Introduction of proposed method:
\begin{itemize}
    \item Another type of synergy that is yet to be explored in HPIs is the task-space synergy, where the motion of the driving joints (residual limb) is mapped to motion of the end-effector (hand).
    \item This task-space synergy can be formulated by utilizing known kinematic information of the human-prosthesis arm and traditional methods used in robotics to define an explicit relationship between the motion of the hand and joints in the arm.
    \item Then, the task-space synergy can be determined as a function of the desired hand motion, and the pose and motion of the residual limb.
    \item Such method would not require any training data, as only physical properties are necessary to explicitly determine the synergy.
    \item
    \item In this paper, such method is explored for the case of elbow prosthesis and forward reaching motion.
    \item By constraining and normalising the desired hand motion, and leveraging the voluntary information that can obtained from the prosthesis user, a task-space synergy-based HPI that can achieve arbitrary point-to-point hand motion is proposed.
    \item The two types of synergy-based HPIs (task-space and joint-space) are experimentally studied for a forward reaching task in isolation from other components used in prosthetic devices to analyse the effects of synergy-based HPIs on task performance and motor behaviour.
    \item Furthermore, these are compared against able-bodied motion and a traditional sEMG based HPI.
\end{itemize}
%
% Notation
%
The following notation is used throughout the paper. The set of real numbers is denoted as $\Real$, the set of positive real numbers is denoted as $\RealPos$. The left hand superscript $\frameOfRef{R}\xv$ is used to indicate the frame of reference $\{R\}$ of the vector $\xv$. The right hand superscript $x^{i}$ is used to indicate the iteration domain, such that $x^{i}$ indicates the $i$th iteration of $x$.

==> old/older/2_formulation_v1.tex <==
%
% Problem formulation
%
\section{Problem formulation}
%
% Formulate in problem in terms of the kinematic analysis
%
\begin{itemize}
    \item The objective is to obtain a synergy for general reaching motion/tasks where the motion of the elbow (prosthesis) is coordinated with the motion of the shoulder (residual limb).
    \item Considering only shoulder and elbow joints. Limited to hand position, no orientation.
    \item From the kinematic analysis of the arm, the following relationship between hand path velocity and joint angular velocities is known
    \begin{equation}
        \pvd = \Jacob(\qv_r,\qv_p)\begin{bmatrix} \qvd_r & \qvd_p \end{bmatrix}^T,
    \end{equation}
    where $\pvd\in\Real^3$ is the hand velocity in task space. $\qv_r$ and $\qvd_r$ represent residual limb joint angular displacement and velocity respectively, for the transhumeral amputation case $\qv_r\in\Real^3$ and $\qvd_r\in\Real^3$. $\qv_p$ and $\qvd_p$ represent prosthesis joint angular displacement and velocity respectively, for the elbow prosthesis case $\qv_r\in\Real$ and $\qvd_r\in\Real$. $\mcl{J}(\qv_r,\qv_p)$ is the arm Jacobian.
    \item With knowledge of the desired hand motion ($\pvd$), it is possible to find a relationship between the residual limb joints and the prosthesis joints angular velocities, $\qvd_r$ and $\qvd_p$ respectively.
    \begin{equation}
        \qvd_p = \Jacob_{p}^{\#}(\qv_r,\qv_p)(\pvd - \Jacob_r(\qv_r,\qv_p)\qvd_r)
    \end{equation}
    $\Jacob_{p}^{\#}(\qv_r,\qv_p)$ is the pseudo-inverse of the Jacobian component related to the prosthesis joint velocities. $\Jacob_r(\qv_r,\qv_p)$ is the Jacobian component related to the residual limb joint velocities.
    \item In the prosthetic case, knowing the desired hand motion $\pvd$ before execution of the task is a challenge as this is only known to the human.
    
    \item 
    \item Reaching motion can be normalized such that the hand path is invariant of the start and end positions \cite{Yang2002}.
    \item Forward reaching motion has been found to be most significantly related to the synergy between shoulder and elbow flexion/extension \cite{Bockemuhl2010}.
    
    \item
    \item By constraining the motion to forward reaching, it is possible to determine the desired path.
    \item This restricts the admissible path to a subset of the full range of able-bodied arm motion, this is a trade-off between practical functionality and full-unconstrained functionality.
    
    
    
    
    \item We can normalize forward reaching motion along the most significant synergy by looking at the planar motion of the arm. Where the plane of motion is formed by the triangle formed by the shoulder and elbow joints, and the hand grasp point.
    
    \begin{figure*}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching1.png}
        \caption{Target reaching example. The green dotted line shows the shortest path to target. The Orange dotted line the forward straight reaching path. Reference frame represented by the subscript $r$, and located at the C7 vertebrae with the $x$ axis pointing forward.}
        \label{fig:reaching1}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching2.png}
        \caption{Simplified geometry for a reaching task by re-positioning the hand. The hand slides across the forward reaching path.}
        \label{fig:reaching2}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/reaching3.png}
        \caption{Definition of the motion direction ($d$) and hand ($h$) frames that determine the forward reaching motion. The direction frame is defined by the triangle created by the shoulder (S), elbow (E), and hand (H) joints and it has its origin at the shoulder joint.}
        \label{fig:reaching3}
    \end{subfigure}
    \caption{Formulation of the forward reaching task and reference motion for the Jacobian-based synergistic prosthesis interface.}\label{fig:reaching}
    \end{figure*}

    \item Then generate the desired forward hand path as a function of the current pose.
    \item Assumptions:
    \begin{itemize}
        \item The angular position and velocity of the residual limb is measurable. IMU-based measurements of residual limb motion have been demonstrated for synergistic elbow prostheses in \cite{Merad2016a}.
        \item Physical properties of the human-prosthesis arm, such as joint-to-joint length, are known.
    \end{itemize}
    \item Formulation:
    \begin{itemize}
        \item Let the origin of the frame of reference ($\{0\}$) be located at the shoulder joint center. The frame of reference is defined as follows:
        \begin{itemize}
            \item $x_0$-axis: unit vector given in the direction from the shoulder joint center to the current hand grasp location.
            \begin{equation}
                ^{0}x_0 = \frac{^{0}\pv}{\|^{0}\pv\|}
            \end{equation}
        \end{itemize}
    \end{itemize}
\end{itemize}

==> old/older/3_synergy_vShort.tex <==
%
% Task-space kinematic synergy
%
\section{A Task-space Kinematic Synergy}
The objective of a task-space kinematic synergy is to determine the motion of the prosthesis given the motion of the residual limb and the desired hand path. However, knowing the exact desired hand path before execution of the task is a challenge as information on the desired target is only known to the prosthesis user. While there exist methods to obtain this information through other interfaces (e.g. brain-machine interfaces \cite{Lew2012}), here, a path-constraint approach is taken to allow the prosthetic user to convey the information of the target prior to commencing the reaching motion. This is done by defining a normalised forward reaching path to be used on any arbitrary point-to-point direction \cite{Yang2002}, such that the user only needs to determine the direction of motion immediately prior to the reaching motion. Due to the normalisation, a shoulder-elbow flexion synergy is sufficient to achieve a forward reaching movement, while the other degrees of freedom in the arm determine which is the forward direction of the reaching movement. While this restricts the admissible path to a subset of the full range of able-bodied arm motion, it is important to highlight the existence of the trade-off between practical functionality and generality of the approach.

\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching1.png}
    \caption{Target reaching example. The green dotted line shows the shortest path to target. The orange dotted line the forward straight reaching path. The reference frame \{R\} has its origin at the shoulder with the $x_r$-axis pointing forward.}
    \label{fig:reaching1}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching2.png}
    \caption{Simplified geometry for a reaching task by re-positioning the hand. The hand slides across the forward reaching path. The $x_r$-$z_r$ plane is parallel to the ground.}
    \label{fig:reaching2}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Figures/reaching3.png}
    \caption{Definition of the direction of motion ($\{D\}$) and hand ($\{H\}$) frames that determine the forward reaching motion. The direction frame is defined by the triangle created by the shoulder (S), elbow (E), and hand (H) joints and it has its origin at the shoulder joint.}
    \label{fig:reaching3}
\end{subfigure}
\caption{Formulation of the forward reaching task and reference motion for the task-space synergy.}
\label{fig:reaching}
\vspace{-13pt}
\end{figure*}

Figure \ref{fig:reaching} presents an example of a target reaching task. By first re-positioning the hand to be aligned with the target on a forward reaching path (Figure \ref{fig:reaching1}), then the synergy can coordinate the motion of prosthetic elbow with that of the residual limb to move the hand linearly towards the target, as if sliding on the path. This is represented in Figure \ref{fig:reaching2}, where the vector from the shoulder joint to the hand ($\rv_{SH}$) defines the direction of the forward reaching motion. Figure \ref{fig:reaching3} presents the proposed simplified geometry, along with frames of reference, used to define the desired hand path.

The methodology followed to achieve the desired hand motion through a task-space kinematic synergy is presented next. Let $\vv\in\Real^3$ be the hand velocity in task-space. $\qv_s$ and $\qvd_s$ are the residual limb joint angular displacement and velocity respectively, for the transhumeral amputation case $\qv_s\in\Real^3$ and $\qvd_s\in\Real^3$. $\qv_e$ and $\qvd_e$ represent prosthesis joint angular displacement and velocity respectively, for the elbow prosthesis case $\qv_e\in\Real$ and $\qvd_e\in\Real$. %$\mcl{J}(\qv_s,\qv_e)$ is the human-prosthetic arm Jacobian.

First, the user pre-positions the hand on the direction of motion path while the prosthesis is disabled, and then enables (or calibrates) the task-space synergy. The enabling can be done through additional interface modalities, such as sEMG, where the user can voluntarily manipulate the signal. Then, in order to obtain the synergy between the shoulder (residual limb) and the hand motion (prosthesis) for a given start position the following steps are taken:
\renewcommand{\labelenumi}{\Alph{enumi}.}
\begin{enumerate}
    \item Determine the forward reaching task direction of motion reference frame (frame $\{D\}$).
    \item Determine the frame transformation ($\transform{D}{R}R$) in order to express shoulder and elbow joint angular displacement with reference to frame $\{D\}$.
    \item Determine the arm Jacobian and the hand motion constraint on $^{D}\dot{x}_h$.
    \item Solve for $\qvd_e$ as a function of $\qv_s$, $\qv_e$, and $\qvd_s$ to determine the elbow motion reference that satisfies the desired task-space synergy.
\end{enumerate}

% \begin{remark}
% It is important to note that while the motion coupling is between the residual limb and the hand, the prosthesis is actuated by the elbow. Thus it is necessary to solve for the elbow motion that will satisfy the desired hand motion. This is done through the arm Jacobian.
% \end{remark}

The following assumptions are used:
\begin{assumption}
    The angular position and velocities of the residual limb are measurable. 
\end{assumption}
\begin{remark}
    Intertial Measurement Unit (IMU)-based measurements of residual limb motion have been demonstrated for synergistic elbow prostheses in \cite{Alshammary2018, Merad2016a}.
\end{remark}
\begin{assumption}
    The joint-to-joint distances of the human-prosthesis arm are known.
\end{assumption}
\begin{remark}
    Joint-to-joint distances of the arm are required to determine the arm Jacobian. Moreover, knowledge of the dimensions of the the user's residual limb and prosthesis, along with measurements of joint position, allow the computation of the hand pose ($\pv$) using forward kinematics.
\end{remark}
The steps of the proposed method to determine the task-space synergy are detailed next.
%
% D frame
%
\subsection{Direction of Motion Reference Frame} 
The direction of motion reference frame determines the direction of the forward reaching task as exemplified in Figure \ref{fig:reaching2}. Let a reference frame (frame $\{R\}$) be located at the center of the shoulder joint with the $x$-axis pointing forward and the $y$-axis upwards w.r.t. the upper body. Let the origin of the direction of motion frame (frame \{D\}) be located at the center of the shoulder joint. The direction of motion frame w.r.t. the reference frame is defined as follows:

The $x_d$-axis is defined by the unit vector given in the direction from the shoulder joint center to the initial hand position $\frameOfRef{R}\pv$, as $\frameOfRef{R}\xv_d = \frac{\frameOfRef{R}\pv}{\|\frameOfRef{R}\pv\|_2}$. The $z_d$-axis is defined by the unit vector perpendicular to the plane given by the S-E-H triangle in the direction of $z_r$, as $\frameOfRef{R}\zv_d =  \frac{ \frameOfRef{R}\rv_{RE} \times \frameOfRef{R}\xv_d }{\|\frameOfRef{R}\rv_{RE} \times \frameOfRef{R}\xv_d\|_2}$. The $y_d$-axis follows the right hand rule. With this the direction of motion reference frame $\{D\}$ is defined and motion of the arm and hand can be expressed with it as reference. This concludes step A. 

%
% Frame transformation
%
\subsection{Frame Transformation} 
Assuming that measured data is obtained in frame $\{R\}$ then it is necessary to transform these angles to the task frame $\{D\}$. This assumption arises from the common use of relative measurements from two IMUs to produce residual limb pose measurements \cite{Alshammary2018, Merad2016a}. This transformation can be performed through the Euler angles ($\alpha$, $\beta$, $\gamma$) in a Y-X-Z sequence. The transformation angles can be obtained as follows:

The first rotation ($\alpha$) is along the $y_r$-axis. $\alpha$ can be obtained from $\frameOfRef{R}\xv_d$, and is defined as $\alpha = \tan^{-1}{\left ( \frac{\frameOfRef{R}\xv_{d,x}}{\frameOfRef{R}\xv_{d,z}} \right )}$, where $\frameOfRef{R}\xv_{d,x}$ and $\frameOfRef{R}\xv_{d,z}$ are the $x$ and $z$ components of $\frameOfRef{R}\xv_{d}$. The second rotation ($\beta$) is along the $x_r$-axis. $\beta$ can be obtained from $\frameOfRef{R}\zv_d$, and is defined as $\beta = \tan^{-1}{\left ( \frac{\frameOfRef{R}\zv_{d,y}}{\frameOfRef{R}\zv_{d,z}} \right )}$. The last rotation ($\gamma$) is along the $z_r$-axis. $\gamma$ can be obtained from $\frameOfRef{R}\xv_d$, and is defined as $\gamma = \tan^{-1}{\left ( \frac{\frameOfRef{R}\xv_{d,y}}{\frameOfRef{R}\xv_{d,x}} \right )}$.

Then the frame transformation is given by
\begin{equation}
    \transform{D}{R}R = R_{y}(\alpha)R_{x}(\beta)R_{z}(\gamma),
\end{equation}
where $R_{x}(\alpha)$ is an $x$-axis standard rotation of the given angle $\alpha$. Thus it is possible to transform arm motion data from the reference frame $\{R\}$ to the task frame $\{D\}$. This concludes step B.

%
% Jacobian
%
\subsection{Arm Jacobian}
By performing the adequate transformations, as previously presented, the forward reaching task can be simplified to a 2D task on the $x-y$ plane of the $D$ frame. This simplifies the kinematics required for the synergy to those of a 2-DOF planar arm. The differential kinematics of the simplified arm are well known and given by \cite{Murray1994}:
\begin{equation}
\label{eq:simpDiffKine}
    \bar{\vv} = \begin{bmatrix} ^{D}\dot{x}_h \\ ^{D}\dot{y}_h \end{bmatrix} = \begin{bmatrix}
    -\ell_{u} S_s - \ell_{l} S_{se} & -\ell_{l} S_{se}\\
    \ell_{u} C_s + \ell_{l} C_{se} & \ell_{l} C_{se}
    \end{bmatrix}\begin{bmatrix} \dot{q}_s \\ \dot{q}_e \end{bmatrix}.
\end{equation}
where $C_s = \cos{(\bar{q}_{s})}$, $S_s = \sin{(\bar{q}_{s})}$, $C_{se} = \cos{(\bar{q}_{s} + \bar{q}_{e})}$, $S_{se} = \sin{(\bar{q}_{s} + \bar{q}_{e})}$, $\bar{q}_{s} = \frameOfRef{D}q_{s}$, and $\bar{q}_{e} = \frameOfRef{D}q_{e}$. $\ell_{u}$and $\ell_{l}$ are the lengths of the upper and lower arm respectively. This concludes step C.

%
% Synergy
%
\subsection{Elbow Motion Reference}
As previously discussed, through the simplification of the task only forward reaching motion is required along the direction of motion plane, i.e. only motion along the $x_d$-axis. This means that it is desired to satisfy the constraint $^{D}\dot{y}_h = 0$. With this constraint in consideration, it is possible to solve for the desired elbow velocity $\dot{q}_e$ from Equation (\ref{eq:simpDiffKine}), such that
\begin{equation}
\label{eq:taskSpaceSynergy}
    \dot{q}_e = -\ell_{l} C^{-1}_{se}(\ell_{u} C_s + \ell_{l} C_{se})\dot{q}_s.
\end{equation}
It is important to note that a singularity exists when $\bar{q}_{s} + \bar{q}_{e} = n\pi/2$, $n = 1, 3, \cdots$; and needs to be properly handled. This concludes step D.

